Visual Concept Connectome (VCC): Open World Concept Discovery and their Interlayer Connections in Deep Models

Understanding what deep network models capture in their learned representations is a fundamental challenge in computer vision. We present a new methodology to understanding such vision models, the Visual Concept Connectome (VCC), which discovers human interpretable concepts and their interlayer connections in a fully unsupervised manner. Our approach simultaneously reveals fine-grained concepts at a layer, connection weightings across all layers and is amendable to global analysis of network structure (e.g., branching pattern of hierarchical concept assemblies). Previous work yielded ways to extract interpretable concepts from single layers and examine their impact on classification, but did not afford multilayer concept analysis across an entire network architecture. Quantitative and qualitative empirical results show the effectiveness of VCCs in the domain of image classification. Also, we leverage VCCs for the application of failure mode debugging to reveal where mistakes arise in deep networks.

==> sec/4_experiments.tex <==

\begin{figure}[t]
    \centering
    \resizebox{0.48\textwidth}{!}{    
    \begin{tikzpicture}[
        every node/.style = {inner sep=0pt},
every label/.append style = {label distance=2pt, align = center},
         sibling distance = 6em,
           level 1/.style = {level distance=5em,anchor=north},
           level 2/.style = {level distance=5em,anchor=north},
           level 3/.style = {level distance=5em,anchor=north},
           ]  
\node[anchor=south,label={[label distance=-0.03cm]left:\rotatebox{90}{Jay}}](class jay)
% class snowmobile
{\includegraphics[width=25mm]{images/connectomes/googlenet_jay_431/class jay.png}}
    child {node[label={[label distance=-0.03cm]left:\rotatebox{90}{inception5b}},label={[xshift=0.5cm,yshift=-0.05cm]above left:{\scriptsize $c_{51}$}}](inception5b jay_concept5){\includegraphics[width=20mm]{images/connectomes/googlenet_jay_431/inception5b jay_concept5.png}} 
    edge from parent[draw=none]} 
    child {node[label={[xshift=0.8cm,yshift=-0.05cm]above left:{\scriptsize $c_{52}$}}](inception5b jay_concept4){\includegraphics[width=20mm]{images/connectomes/googlenet_jay_431/inception5b jay_concept4.png}} 
        edge from parent[draw=none]
        child {node[xshift=1.05cm,label={[label distance=-0.03cm]left:\rotatebox{90}{inception4c}},label={[xshift=0.7cm,yshift=-0.05cm]above left:{\scriptsize $c_{41}$}}](inception4c jay_concept2){\includegraphics[width=20mm]{images/connectomes/googlenet_jay_431/inception4c jay_concept2.png}} 
        edge from parent[draw=none]}
        child {node[xshift=1.05cm,label={[xshift=-0.7cm,yshift=-0.05cm]above right:{\scriptsize $c_{42}$}}](inception4c jay_concept5) {\includegraphics[width=20mm]{images/connectomes/googlenet_jay_431/inception4c jay_concept5.png}} 
        edge from parent[draw=none]
            child {node[xshift=1.05cm,label={[label distance=-0.0cm]left:\rotatebox{90}{conv3}},label={[xshift=0.5cm,yshift=-0.05cm]above left:{\scriptsize $c_{31}$}}](conv3 jay_concept3){\includegraphics[width=20mm]{images/connectomes/googlenet_jay_431/conv3 jay_concept3.png}} 
            edge from parent[draw=none]}
            child {node[xshift=1.05cm,label={[xshift=-0.9cm,yshift=-0.05cm]above right:{\scriptsize $c_{32}$}}](conv3 jay_concept2){\includegraphics[width=20mm]{images/connectomes/googlenet_jay_431/conv3 jay_concept2.png}} 
            edge from parent[draw=none]}
            child {node[xshift=1.05cm,label={[xshift=-0.5cm,yshift=-0.05cm]above right:{\scriptsize $c_{33}$}}](conv3 jay_concept1){\includegraphics[width=20mm]{images/connectomes/googlenet_jay_431/conv3 jay_concept1.png}} 
            edge from parent[draw=none]}
            }
        child {node[xshift=1.05cm,label={[xshift=1.06cm,yshift=-0.05cm]above left:{\scriptsize $c_{43}$}}](inception4c jay_concept1){\includegraphics[width=20mm]{images/connectomes/googlenet_jay_431/inception4c jay_concept1.png}} 
            edge from parent[draw=none]} 
        child {node[xshift=1.05cm,label={[xshift=-0.5cm,yshift=-0.05cm]above right:{\scriptsize $c_{44}$}}](inception4c jay_concept3){\includegraphics[width=20mm]{images/connectomes/googlenet_jay_431/inception4c jay_concept3.png}} 
            edge from parent[draw=none]}
            } 
    child {node[label={[xshift=-0.8cm,yshift=-0.05cm]above right:{\scriptsize $c_{53}$}}](inception5b jay_concept3){\includegraphics[width=20mm]{images/connectomes/googlenet_jay_431/inception5b jay_concept3.png}} edge from parent[draw=none]} 
    child {node[label={[xshift=-0.5cm,yshift=-0.05cm]above right:{\scriptsize $c_{54}$}}](inception5b jay_concept2){\includegraphics[width=20mm]{images/connectomes/googlenet_jay_431/inception5b jay_concept2.png}} edge from parent[draw=none]
            };
% ARROWS
\begin{scope}[on background layer]
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(590)] ($ (conv3 jay_concept3.north) - (0,0.2) $) -- ( $ (inception4c jay_concept2.south) + (0,0.25) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(457)] ($ (conv3 jay_concept3.north) - (0,0.2) $) -- ( $ (inception4c jay_concept5.south) + (0,0.25) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(343)] ($ (inception4c jay_concept2.north) - (0,0.2) $) -- ( $ (inception5b jay_concept5.south) + (0,0.25) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(308)] ($ (inception4c jay_concept2.north) - (0,0.2) $) -- ( $ (inception5b jay_concept2.south) + (0,0.25) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(357)] ($ (inception4c jay_concept5.north) - (0,0.2) $) -- ( $ (inception5b jay_concept4.south) + (0,0.25) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(734)] ($ (conv3 jay_concept2.north) - (0,0.2) $) -- ( $ (inception4c jay_concept1.south) + (0,0.25) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(617)] ($ (conv3 jay_concept2.north) - (0,0.2) $) -- ( $ (inception4c jay_concept2.south) + (0,0.25) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(510)] ($ (conv3 jay_concept2.north) - (0,0.2) $) -- ( $ (inception4c jay_concept5.south) + (0,0.25) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(329)] ($ (inception4c jay_concept1.north) - (0,0.2) $) -- ( $ (inception5b jay_concept5.south) + (0,0.25) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(361)] ($ (inception4c jay_concept1.north) - (0,0.2) $) -- ( $ (inception5b jay_concept4.south) + (0,0.25) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(329)] ($ (inception4c jay_concept1.north) - (0,0.2) $) -- ( $ (inception5b jay_concept3.south) + (0,0.25) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(312)] ($ (inception4c jay_concept1.north) - (0,0.2) $) -- ( $ (inception5b jay_concept2.south) + (0,0.25) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(547)] ($ (conv3 jay_concept1.north) - (0,0.2) $) -- ( $ (inception4c jay_concept3.south) + (0,0.25) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(675)] ($ (conv3 jay_concept1.north) - (0,0.2) $) -- ( $ (inception4c jay_concept1.south) + (0,0.25) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(657)] ($ (conv3 jay_concept1.north) - (0,0.2) $) -- ( $ (inception4c jay_concept2.south) + (0,0.25) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(520)] ($ (conv3 jay_concept1.north) - (0,0.2) $) -- ( $ (inception4c jay_concept5.south) + (0,0.25) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(229)] ($ (inception4c jay_concept3.north) - (0,0.2) $) -- ( $ (inception5b jay_concept5.south) + (0,0.25) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(291)] ($ (inception4c jay_concept3.north) - (0,0.2) $) -- ( $ (inception5b jay_concept4.south) + (0,0.25) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(0)] ($(inception5b jay_concept5.north) - (0,0.3) $) -- ( $ (class jay.south) + (0,0.3) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(0)] ($(inception5b jay_concept4.north) - (0,0.3) $) -- ( $ (class jay.south) + (0,0.3) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(0)] ($(inception5b jay_concept3.north) - (0,0.3) $) -- ( $ (class jay.south) + (0,0.3) $);
\draw[line width=0.7mm,,-,/pgfplots/color of colormap=(0)] ($(inception5b jay_concept2.north) - (0,0.3) $) -- ( $ (class jay.south) + (0,0.3) $);
\end{scope}
    \end{tikzpicture}
}\vspace{-0.3cm}
\caption{\textcolor{blue}{A VCC for three selected layers of a GoogLeNet model~\cite{szegedy2015going} targeting recognition of class ``Jay". Darker lines denote stronger connection weights.} 
} \vspace{-0.5cm}
\end{figure}\label{fig:goog_jay} 

%\vspace{-0.2cm}
\section{Experiments}\label{sec:experiments}
%This section unfolds in four subsections. (1) Implementation details are documented, Sec.~\ref{sec:implementation_details}. (2) The three main technical components of VCC construction are validated empirically, Sec.~\ref{sec:validation}. VCCs are used to
%In this section, we first describe the implementation details of the approach. We then quantitatively validate the three main components of the proposed methodology. Finally, we use VCC's 
%interpret the concepts and their interlayer connections across (3) architectures, Sec.~\ref{sec:architectures} and (4) training objectives, Sec.~\ref{sec:tasks}.


\subsection{Implementation details}\label{sec:implementation_details}

% The number of clusters during the segment proposal stage, $k_n$, is chosen based on the Elbow Criterion\cite{kodinariya2013review}. For object recognition, we found that $k_n=2$ for the vast majority of images. We hypothesize that this is because at the final layer of the model, the representations are generally clustered into `foreground' and `background' (\ie object and non-object) regions. 
% The number of clusters during the segment proposal stage are all chosen using the silhouette method.
For evaluation we use ResNet50~\cite{he2016deep}, VGG16~\cite{simonyan2014very}, MobileNetv3~\cite{howard2019searching}, ViT-b~\cite{vaswani2017attention} and MViT~\cite{fan2021multiscale}, which captures a broad range of popular architectures.
%and corresponding four layers to generate VCCs (as named in PyTorch modules): ResNet50~\cite{he2016deep}: \{\textit{Layer1}, \textit{Layer2}, \textit{Layer3}, \textit{Layer4}\}, GoogLeNet~\cite{szegedy2015going}: \{\textit{Layer1}, \textit{Layer2}, \textit{Layer3}, \textit{Layer4}\}, VGG16~\cite{simonyan2014very}: \{\textit{8}, \textit{15}, \textit{22}, \textit{29}\}, MobileNetv2~\cite{sandler2018mobilenetv2}: \{\textit{4}, \textit{11}, \textit{14}, \textit{18}\}, MViT~\cite{fan2021multiscale}: \{\textit{1}, \textit{3}, \textit{5}, \textit{9}\}, ViT-b~\cite{vaswani2017attention}: \{\textit{2}, \textit{5}, \textit{8}, \textit{10}\}. 
For each model, we select four layers with approximately even spacing across the model (\ie to capture low, mid and high level concepts, with exact layers in the supplement); we also include the last feature layer before the fully connected layer to probe concepts closest to the model output. Here, we consider only four layer VCCs for visualization ease.

% \textcolor{blue}{MK & KGD: We suggest to move the clustering details to the supplement.}

% Following previous work~\cite{ghorbani2019towards}, during the concept discovery clustering, $\mathsf{C}^{con}$, we over-cluster and then prune to ensure that fewer concepts will be missed. We follow the pruning protocol from~\cite{ghorbani2019towards}: We choose the number of clusters to be $k_{m}=25$ in the concept discovery step, remove the clusters that have 75\% of segments coming from the same image, and clusters with less than $\delta * |\mathbf{M}_i|$ segments belonging to it (\ie a fraction of the total segment dataset for that layer), where $\delta = \frac{1}{16}$. The Euclidean distance is used for all clustering steps.

Following~\cite{kim2018interpretability,ghorbani2019towards}, we perform a two-sided t-test on ITCAV scores for multiple runs of the same concept vs. different random datasets to remove statistically insignificant scores. %, and
Also following~\cite{kim2018interpretability,ghorbani2019towards}, we 
randomly sample from the Broden dataset~\cite{bau2017network} to get the images, $\bm{\mathcal{I}}_{rnd}$ (Sec.~\ref{sec:itcav}), used in statistical testing and CAV training.
%the random images, $\bm{\mathcal{I}}_{rnd}$ (Sec.~\ref{sec:itcav}), used in the statistical testing and CAV training are randomly sampled from the Broden dataset~\cite{bau2017network}. 
A four-layer VCC takes \textcolor{blue}{15 minutes} on average to generate \todo{in unoptimized code} on an NVIDIA Quadro RTX 6000 GPU (24GB). The supplement has more implementation details and VCCs for more layers, models, and additional datasets~\cite{WahCUB_200_2011}.
%The supplement includes the clustering hyperparameters, VCCs with additional models, layer settings, timings to generate VCCs, additional details on the statistical testing and exact layers specifications.





\subsection{VCC component validation}\label{sec:validation}
%We now validate the three main components of the proposed methodology: (1) segment proposals via divisive clustering  (Sec.~\ref{sec:validateSegment}), (2) layer-wise concept discovery via clustering of segment features (Sec.~\ref{sec:validateConcept}), and (3) inter-layer concept connection weights via ITCAV (Sec.~\ref{sec:validateITCAV}). 
%For the segment validation, we demonstrate that our approach follows a model's receptive field spatial support more closely than the baseline, ACE~\cite{ghorbani2019towards}. For the concept discovery validation, we show that the concept centroid directions are meaningful as they have a greater impact on model performance than random directions when perturbed in feature space. To validate ITCAV, we demonstrate a correlation between the strength of the ITCAV weights from a concept to the output, and the probability of observing the target class.










%\subsubsection{Segment proposal validation} \label{sec:validateSegment}
\textbf{Segment proposal validation.} Our approach segments concepts based on the feature space of a given layer to allow us to capture concepts across multiple layers (Sec.~\ref{sec:divisive_cluster}). Correspondingly, the spatial support of valid segments at a layer should follow the receptive field (RF) of filters at that layer, because the segments are constrained by the filters from which they are derived. For comparison, we consider ACE~\cite{ghorbani2019towards}, which uses a layer independent feature (color) limited to the input image for segmentation to discover concepts at a single layer for a single model. Being directly related to the features at a layer, our approach should produce concepts that better respect the RF at that layer compared to the baseline, whose features are independent of layer (\eg at the early layers of a ConvNet, the RF is small and intuitively the patch proposals should be smaller as well, and conversely for the later layers). 







\begin{figure} [t]
	\begin{center}
     \centering 
\resizebox{0.48\textwidth}{!}{
\hspace{0.1cm}
\begin{tikzpicture} 
                 \begin{axis}[
                 line width=1.0,
                 % title={Branching Factor},
                 title style={at={(axis description cs:0.5,1.2)},anchor=north,font=\normalsize},
                 % xlabel={Top-k \% Units Masked},
                 ylabel={Branching Factor},
                 xmin=0.5, xmax=4.5,
                 ymin=0, ymax=8,
                 xtick={1,2,3,4},
                %  ytick={30, 35, 40, 45, 50, 55, 60, 65, 70},
                 x tick label style={font=\tiny, rotate=0, anchor=north},
                 y tick label style={font=\tiny},
                 x label style={at={(axis description cs:0.5,0.09)},anchor=north,font=\small},
                 y label style={at={(axis description cs:0.2,.5)},anchor=south,font=\small},
                 width=6.5cm,
                 height=4.0cm, % height=4.3cm, 
                 ymajorgrids=false,
                 xmajorgrids=false,
                 major grid style={dotted,green!20!black},
                 % legend columns=2,
                 % legend style={
                 %  nodes={scale=0.7, transform shape},
                 %  cells={anchor=west},
                 %  legend style={at={(0.5,1)},anchor=north,row sep=0.01pt}, font =\small}
             ]

             % \addlegendentry{GoogLeNet}
             % \addplot[line width=0.9pt, mark size=1.6pt, color=cyan, mark=square,error bars/.cd, y dir=both, y explicit,]
             %         coordinates {(1, 2.404)
             %                      (2, 1.127)
             %                      (3, 2.782)
             %                      (4, 3.74)};
            % \addlegendentry{ResNet50}
            \addplot[line width=0.9pt, mark size=1.6pt, color=cyan, mark=o,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 5.484)
                                  (2, 4.945)
                                  (3, 2.799)
                                  (4, 2.915)};
            % \addlegendentry{VGG16}
            \addplot[line width=0.9pt, mark size=1.6pt, color=cyan, mark=diamond,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 6.765)
                                  (2, 6.249)
                                  (3, 4.599)
                                  (4, 1.696)};
            % \addlegendentry{MobileNet-v3}
            \addplot[line width=0.9pt, mark size=1.6pt, color=cyan, mark=triangle,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 7.102)
                                  (2, 5.175)
                                  (3, 4.3)
                                  (4, 1.149)};
            % \addlegendentry{MViT}
            \addplot[line width=0.9pt, mark size=1.6pt, color=red, mark=x,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 5.659)
                                  (2, 5.886)
                                  (3, 6.585)
                                  (4, 2.043)};
            % \addlegendentry{ViT}
            \addplot[line width=0.9pt, mark size=1.6pt, color=red, mark=+,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 2.967)
                                  (2, 2.044)
                                  (3, 3.337)
                                  (4, 1.66)};                                  
              \end{axis}
\end{tikzpicture}
\hspace{0.1cm}
\begin{tikzpicture} 
                  \begin{axis}[
                 line width=1.0,
                 % title={Concepts},
                 title style={at={(axis description cs:0.5,1.2)},anchor=north,font=\normalsize},
                 % xlabel={Layer},
                 ylabel={Number of Concepts},
                 xmin=0.5, xmax=4.5,
                 ymin=1.5, ymax=12.5,
                 xtick={1,2,3,4},
                %  ytick={30, 35, 40, 45, 50, 55, 60, 65, 70},
                 x tick label style={font=\tiny, rotate=0, anchor=north},
                 y tick label style={font=\tiny},
                 x label style={at={(axis description cs:0.5,0.09)},anchor=north,font=\small},
                 y label style={at={(axis description cs:0.2,.5)},anchor=south,font=\small},
                 width=6.5cm,
                 height=4.0cm, % height=4.3cm, 
                 ymajorgrids=false,
                 xmajorgrids=false,
                 major grid style={dotted,green!20!black},
                 legend columns=2,
                 legend style={
                  nodes={scale=0.7, transform shape},
                  cells={anchor=west},
                  legend style={at={(0.5,1)},anchor=north,row sep=0.01pt}, font =\small}
             ]

             % \addlegendentry{GoogLeNet}
             % \addplot[line width=0.9pt, mark size=1.6pt, color=cyan, mark=square,error bars/.cd, y dir=both, y explicit,]
             %         coordinates {(1, 3.46)
             %                      (2, 2.74)
             %                      (3, 4.04)
             %                      (4, 4.7)};
            % \addlegendentry{ResNet50}
            \addplot[line width=0.9pt, mark size=1.6pt, color=cyan, mark=o,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1,10.447)
                                  (2, 8)
                                  (3, 5.106)
                                  (4, 2.957)};
            % \addlegendentry{VGG16}
            \addplot[line width=0.9pt, mark size=1.6pt, color=cyan, mark=diamond,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 11.174)
                                  (2, 9.348)
                                  (3, 6.348)
                                  (4, 3.087)};
            % \addlegendentry{MobileNet-v2}
            \addplot[line width=0.9pt, mark size=1.6pt, color=cyan, mark=triangle,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 12.255)
                                  (2, 9.532)
                                  (3, 6.936)
                                  (4, 2.404)};
            % \addlegendentry{MViT}
            \addplot[line width=0.9pt, mark size=1.6pt, color=red, mark=x,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 11.872)
                                  (2, 9.957)
                                  (3, 6.83)
                                  (4, 2.191)};
            % \addlegendentry{ViT}
            \addplot[line width=0.9pt, mark size=1.6pt, color=red, mark=+,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 7.957)
                                  (2, 5.596)
                                  (3, 5.766)
                                  (4, 2.298)};                                  
              \end{axis}
\end{tikzpicture}}
\resizebox{0.48\textwidth}{!}{
\hspace{0.1cm}
% \vspace{-0.2}
\begin{tikzpicture}
                 \begin{axis}[
                 line width=1.0,
                 % title={Branching Factor},
                 title style={at={(axis description cs:0.5,1.2)},anchor=north,font=\normalsize},
                 xlabel={Layer},
                 ylabel={Edge Weight Average},
                 xmin=0.5, xmax=4.5,
                 ymin=0, ymax=1,
                 xtick={1,2,3,4},
                %  ytick={30, 35, 40, 45, 50, 55, 60, 65, 70},
                 x tick label style={font=\tiny, rotate=0, anchor=north},
                 y tick label style={font=\tiny},
                 x label style={at={(axis description cs:0.5,0.15)},anchor=north,font=\small},
                 y label style={at={(axis description cs:0.2,.5)},anchor=south,font=\small},
                 width=6.5cm,
                 height=4.0cm, % height=4.3cm, 
                 ymajorgrids=false,
                 xmajorgrids=false,
                 major grid style={dotted,green!20!black},
                 legend columns=2,
                 legend style={
                  nodes={scale=0.7, transform shape},
                  cells={anchor=west},
                  legend style={at={(0.5,1)},anchor=north,row sep=0.01pt}, font =\small}
             ]

             % \addlegendentry{GoogLeNet}
             % \addplot[line width=0.9pt, mark size=1.6pt, color=cyan, mark=square,error bars/.cd, y dir=both, y explicit,]
             %         coordinates {(1, 0.429)
             %                      (2, 0.412)
             %                      (3, 0.674)
             %                      (4, 0.98)};
            % \addlegendentry{ResNet50}
            \addplot[line width=0.9pt, mark size=1.6pt, color=cyan, mark=o,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 0.414)
                                  (2, 0.554)
                                  (3, 0.476)
                                  (4, 0.917)};
            % \addlegendentry{VGG16}
            \addplot[line width=0.9pt, mark size=1.6pt, color=cyan, mark=diamond,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 0.329)
                                  (2, 0.272)
                                  (3, 0.429)
                                  (4, 0.801)};
            % \addlegendentry{MobileNet-v2}
            \addplot[line width=0.9pt, mark size=1.6pt, color=cyan, mark=triangle,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 0.5)
                                  (2, 0.498)
                                  (3, 0.623)
                                  (4, 0.75)};
            % \addlegendentry{MViT}
            \addplot[line width=0.9pt, mark size=1.6pt, color=red, mark=x,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 0.552)
                                  (2, 0.384)
                                  (3, 0.579)
                                  (4, 0.908)};
            % \addlegendentry{ViT}
            \addplot[line width=0.9pt, mark size=1.6pt, color=red, mark=+,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 0.471)
                                  (2, 0.529)
                                  (3, 0.395)
                                  (4, 0.755)};                                  
              \end{axis}
\end{tikzpicture}
\hspace{0.1cm}
\begin{tikzpicture} 
                  \begin{axis}[
                 line width=1.0,
                 % title={Branching Factor},
                 title style={at={(axis description cs:0.5,1.2)},anchor=north,font=\normalsize},
                 xlabel={Layer},
                 ylabel={Edge Weight Variance},
                 xmin=0.5, xmax=4.5,
                 ymin=0, ymax=0.03,
                 xtick={1,2,3,4},
                %  ytick={30, 35, 40, 45, 50, 55, 60, 65, 70},
                 x tick label style={font=\tiny, rotate=0, anchor=north},
                 y tick label style={font=\tiny},
                 x label style={at={(axis description cs:0.5,0.15)},anchor=north,font=\small},
                 y label style={at={(axis description cs:0.2,.5)},anchor=south,font=\small},
                 width=6.5cm,
                 height=4.0cm, % height=4.3cm, 
                 ymajorgrids=false,
                 xmajorgrids=false,
                 major grid style={dotted,green!20!black},
                    legend columns=2,
                 legend style={
                  nodes={scale=0.7, transform shape},
                  cells={anchor=west},
                  legend style={at={(0.405,1)},anchor=north,row sep=0.01pt}, font =\small}
             ]

             % \addlegendentry{GoogLeNet}
             % \addplot[line width=0.9pt, mark size=1.6pt, color=cyan, mark=square,error bars/.cd, y dir=both, y explicit,]
             %         coordinates {(1, 0.002)
             %                      (2, 0.003)
             %                      (3, 0.009)
             %                      (4, 0.003)};
            \addlegendentry{ResNet50}
            \addplot[line width=0.9pt, mark size=1.6pt, color=cyan, mark=o,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 0.003)
                                  (2, 0.007)
                                  (3, 0.01)
                                  (4, 0.007)};
                \addlegendentry{MViT}
            \addplot[line width=0.9pt, mark size=1.6pt, color=red, mark=x,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 0.003)
                                  (2, 0.003)
                                  (3, 0.005)
                                  (4, 0.016)};
                \addlegendentry{VGG16}
            \addplot[line width=0.9pt, mark size=1.6pt, color=cyan, mark=diamond,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 0.008)
                                  (2, 0.013)
                                  (3, 0.007)
                                  (4, 0.003)};
            \addlegendentry{ViT}
            \addplot[line width=0.9pt, mark size=1.6pt, color=red, mark=+,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 0.011)
                                  (2, 0.007)
                                  (3, 0.008)
                                  (4, 0.028)};          
            \addlegendentry{MobileNet-v3}
            \addplot[line width=0.9pt, mark size=1.6pt, color=cyan, mark=triangle,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(1, 0.008)
                                  (2, 0.008)
                                  (3, 0.006)
                                  (4, 0.004)};
  
                             
              \end{axis}
\end{tikzpicture}
}
\end{center}
\vspace{-0.7cm}
\caption{Graph metrics for the VCCs generated for various ConvNet and transformer architectures. 
% Values are averaged over 50 randomly selected ImageNet~\cite{deng2009imagenet} classes. 
%The number of concepts varies at early and middle layers but converges to around five concepts in the final layer. The average edge weight and edge variance are also less strong and more diverse, respectively, in the final layers for transformer architectures than for CNNs.
}\label{fig:cnn_trans}
\vspace{-0.5cm}
\end{figure}

%We now validate the image segment proposal via divise clustering method as described in Sec.~\ref{sec:divisive_cluster}. 
%Unlike ACE~\cite{ghorbani2019towards}, which discovers concepts at a single layer for a single model, our goal is to be able to connect concepts at multiple layers in a diverse range of models. We therefore we segment concepts based on the feature space of a given layer. contrasting the RGB superpixel method in the baseline ACE~\cite{ghorbani2019towards}. Being directly related to the features at a layer, our approach should produce concepts that better respect the receptive field at that layer compared to the baseline, whose features are independent of layer (\eg at the early layers of a CNN, the receptive field is small and intuitively the patch proposals should be smaller as well, and conversely for the later layers). 

% better respect (1) the receptive field at that layer (\eg at the first few layers of a convolutional network, the receptive field is very small and intuitively the patch proposals should be a similar size as well) and (2) the boundaries of semantically meaningful image regions at a given layer (\eg one would expect segment boundaries between different colors and textures at earlier layers, while boundaries should exist between objects at later layers). 

Figure~\ref{fig:segment_concept_validation} (left) shows the average concept size (in terms of the ratio of segment pixels to the entire image) vs. the RF at the corresponding layer for three different models: (1) ResNet50~\cite{he2016deep}, (2) VGG16~\cite{simonyan2014very} and (3) ViT-b~\cite{dosovitskiy2020image} (note we use mean attention distance instead of receptive field for ViT-b). While the baseline~\cite{ghorbani2019towards} produces segments with sizes invariant to the layer analyzed, our approach produces segments with image sizes that scale with the RF.
Additional results with other models (including transformers) are given in the supplement, which further support this observation. Overall, it is expected by design and we find that our segment proposals follow RFs at each layer.






%\subsubsection{Concept validation} \label{sec:validateConcept}
\textbf{Concept fidelity.} Concept fidelity measures the meaningfulness of the discovered concepts with respect to the target model. This confirms that the discovered concepts are faithful to the model. While other work focuses on single layer concept fidelity~\cite{kim2018interpretability,ghorbani2019towards,fel2023craft}, we measure the effect on a model's performance when suppressing the encoding of concepts as the information propagates through the model. The expectation is that suppressing the discovered concepts should result in a quicker decrease in performance compared to a non-concept direction (\eg a randomly selected direction) as the amount of suppression gets larger. For a given model and category, we compute the concepts at various layers using our method (Sec.~\ref{sec:concept_discovery_clustering}). We perform concept suppression for a given image, $\bm{\mathcal{I}}^i$, at a given layer, $j$, for concept $\textbf{q}_j$, according to $\textbf{z}^i_j = \textbf{z}^i_j -\epsilon \cdot \textbf{q}_j \big/ ||\textbf{q}_j||_2$,
% \begin{equation}
%     \textbf{z}^i_j = \textbf{z}^i_j -\epsilon \cdot \textbf{q}_j \big/ ||\textbf{q}_j||_2,
% \end{equation}
where $\epsilon$ controls the degree of perturbation. If the concepts discovered are meaningful, then the accuracy for the model's target class should decrease faster compared to random perturbations, $\mathbf{q}_{rnd}$, as $\epsilon$ increases.  

Figure~\ref{fig:segment_concept_validation} (right) has concept suppression results averaged over 50 randomly selected ImageNet~\cite{deng2009imagenet} classes (documented in the supplement), where a concept is randomly chosen to be suppressed at each layer (we use the same four layers given in Sec.~\ref{sec:implementation_details}). Note that the $\epsilon$ values required to reduce the model accuracy to zero differs by model; so, we scale the $\epsilon$ values to $[0,1]$ for visualization purposes. For all models, it is seen that perturbing in the opposite direction of a recovered concept more severely impacts the accuracy than a random perturbation. 
% The effect is seen in more compact form in Fig.~\ref{fig:segment_concept_validation} (bottom), where area under curve (AUC) of the accuracy is decreased most when perturbing opposite the direction of a discovered concept. These results support the claim that the concept directions discovered via the segment proposal (Sec.~\ref{sec:divisive_cluster}), and then followed by the layer-wise concept discovery (Sec.~\ref{sec:concept_discovery_clustering}), are meaningful. 






\begin{figure}[t]
    \centering
    \resizebox{0.48\textwidth}{!}{    
    \begin{tikzpicture}[
        every node/.style = {inner sep=0pt},
every label/.append style = {label distance=2pt, align = center},
         sibling distance = 4.75em,
           level 1/.style = {level distance=6em,anchor=north},
           level 2/.style = {level distance=5.5em,anchor=north},
           level 3/.style = {level distance=5em,anchor=north},
           ]  
\node[anchor=south, label=ResNet50](class tow_truck)
% \node[anchor=south, label=A Visual Concept Connectome]
% class teapot
{\includegraphics[width=25mm]{images/connectomes/new/r50_tow_truck/class tow_truck.png}}
    child {node[label={[label distance=-0.03cm]left:\rotatebox{90}{Late Layer}}](layer4 tow_truck_concept1){\includegraphics[width=16mm]{images/connectomes/new/r50_tow_truck/layer4 tow_truck_concept1.png}} 
        edge from parent[draw=none]} 
    child {node[](layer4 tow_truck_concept2){\includegraphics[width=16mm]{images/connectomes/new/r50_tow_truck/layer4 tow_truck_concept2.png}} 
        edge from parent[draw=none]} 
    child {node[](layer4 tow_truck_concept3){\includegraphics[width=16mm]{images/connectomes/new/r50_tow_truck/layer4 tow_truck_concept3.png}} 
        edge from parent[draw=none]
        child {node[xshift=-0.84cm,label={[label distance=-0.03cm]left:\rotatebox{90}{Mid-Layer}}](layer3 tow_truck_concept1){\includegraphics[width=16mm]{images/connectomes/new/r50_tow_truck/layer3 tow_truck_concept1.png}} 
            edge from parent[draw=none]}
        child {node[xshift=-0.84cm](layer3 tow_truck_concept4){\includegraphics[width=16mm]{images/connectomes/new/r50_tow_truck/layer3 tow_truck_concept4.png}} 
            edge from parent[draw=none]} 
        child {node[xshift=-0.84cm](layer3 tow_truck_concept5) {\includegraphics[width=16mm]{images/connectomes/new/r50_tow_truck/layer3 tow_truck_concept5.png}}
            edge from parent[draw=none]} 
            } 
    child {node[](layer4 tow_truck_concept4){\includegraphics[width=16mm]{images/connectomes/new/r50_tow_truck/layer4 tow_truck_concept4.png}} edge from parent[draw=none]};
% ARROWS
\begin{scope}[on background layer]
% \draw[line width=0.4375mm,-,/pgfplots/color of colormap=(563)] ($ (layer1 tow_truck_concept10.north) - (0, 0.2) $) -- ( $ (layer2 tow_truck_concept3.south) + (0, 0.25) $);
% \draw[line width=0.43235294117647066mm,-,/pgfplots/color of colormap=(568)] ($ (layer1 tow_truck_concept10.north) - (0, 0.2) $) -- ( $ (layer2 tow_truck_concept5.south) + (0, 0.25) $);
% \draw[line width=0.6318181818181816mm,-,/pgfplots/color of colormap=(369)] ($ (layer2 tow_truck_concept3.north) - (0, 0.2) $) -- ( $ (layer3 tow_truck_concept6.south) + (0, 0.25) $);
% \draw[line width=0.6117647058823528mm,-,/pgfplots/color of colormap=(389)] ($ (layer2 tow_truck_concept3.north) - (0, 0.2) $) -- ( $ (layer3 tow_truck_concept2.south) + (0, 0.25) $);
% \draw[line width=0.6384615384615384mm,-,/pgfplots/color of colormap=(362)] ($ (layer2 tow_truck_concept3.north) - (0, 0.2) $) -- ( $ (layer3 tow_truck_concept4.south) + (0, 0.25) $);
% \draw[line width=0.6454545454545454mm,-,/pgfplots/color of colormap=(355)] ($ (layer2 tow_truck_concept3.north) - (0, 0.2) $) -- ( $ (layer3 tow_truck_concept1.south) + (0, 0.25) $);
% \draw[line width=0.4mm,-,/pgfplots/color of colormap=(600)] ($ (layer2 tow_truck_concept5.north) - (0, 0.2) $) -- ( $ (layer3 tow_truck_concept2.south) + (0, 0.25) $);
% \draw[line width=0.4999999999999999mm,-,/pgfplots/color of colormap=(501)] ($ (layer2 tow_truck_concept5.north) - (0, 0.2) $) -- ( $ (layer3 tow_truck_concept1.south) + (0, 0.25) $);
% \draw[line width=0.44749999999999995mm,-,/pgfplots/color of colormap=(553)] ($ (layer1 tow_truck_concept4.north) - (0, 0.2) $) -- ( $ (layer2 tow_truck_concept3.south) + (0, 0.25) $);
% \draw[line width=0.39411764705882363mm,-,/pgfplots/color of colormap=(606)] ($ (layer1 tow_truck_concept4.north) - (0, 0.2) $) -- ( $ (layer2 tow_truck_concept5.south) + (0, 0.25) $);
% \draw[line width=0.44750000000000006mm,-,/pgfplots/color of colormap=(553)] ($ (layer1 tow_truck_concept11.north) - (0, 0.2) $) -- ( $ (layer2 tow_truck_concept3.south) + (0, 0.25) $);
% \draw[line width=0.5920000000000001mm,-,/pgfplots/color of colormap=(408)] ($ (layer1 tow_truck_concept11.north) - (0, 0.2) $) -- ( $ (layer2 tow_truck_concept6.south) + (0, 0.25) $);
% \draw[line width=0.5236842105263158mm,-,/pgfplots/color of colormap=(477)] ($ (layer1 tow_truck_concept11.north) - (0, 0.2) $) -- ( $ (layer2 tow_truck_concept7.south) + (0, 0.25) $);
% \draw[line width=0.4117647058823529mm,-,/pgfplots/color of colormap=(589)] ($ (layer1 tow_truck_concept11.north) - (0, 0.2) $) -- ( $ (layer2 tow_truck_concept5.south) + (0, 0.25) $);
% \draw[line width=0.6636363636363635mm,-,/pgfplots/color of colormap=(337)] ($ (layer2 tow_truck_concept6.north) - (0, 0.2) $) -- ( $ (layer3 tow_truck_concept6.south) + (0, 0.25) $);
% \draw[line width=0.5764705882352941mm,-,/pgfplots/color of colormap=(424)] ($ (layer2 tow_truck_concept6.north) - (0, 0.2) $) -- ( $ (layer3 tow_truck_concept2.south) + (0, 0.25) $);
% \draw[line width=0.5384615384615384mm,-,/pgfplots/color of colormap=(462)] ($ (layer2 tow_truck_concept6.north) - (0, 0.2) $) -- ( $ (layer3 tow_truck_concept4.south) + (0, 0.25) $);
% \draw[line width=0.6090909090909091mm,-,/pgfplots/color of colormap=(391)] ($ (layer2 tow_truck_concept7.north) - (0, 0.2) $) -- ( $ (layer3 tow_truck_concept6.south) + (0, 0.25) $);
% \draw[line width=0.5441176470588235mm,-,/pgfplots/color of colormap=(456)] ($ (layer2 tow_truck_concept7.north) - (0, 0.2) $) -- ( $ (layer3 tow_truck_concept2.south) + (0, 0.25) $);
% \draw[line width=0.55mm,-,/pgfplots/color of colormap=(450)] ($ (layer2 tow_truck_concept7.north) - (0, 0.2) $) -- ( $ (layer3 tow_truck_concept4.south) + (0, 0.25) $);
% \draw[line width=0.5863636363636363mm,-,/pgfplots/color of colormap=(414)] ($ (layer2 tow_truck_concept7.north) - (0, 0.2) $) -- ( $ (layer3 tow_truck_concept1.south) + (0, 0.25) $);
% \draw[line width=0.3775mm,-,/pgfplots/color of colormap=(623)] ($ (layer1 tow_truck_concept2.north) - (0, 0.2) $) -- ( $ (layer2 tow_truck_concept3.south) + (0, 0.25) $);
% \draw[line width=0.376470588235294mm,-,/pgfplots/color of colormap=(624)] ($ (layer1 tow_truck_concept2.north) - (0, 0.2) $) -- ( $ (layer2 tow_truck_concept5.south) + (0, 0.25) $);
% \draw[line width=0.612mm,-,/pgfplots/color of colormap=(388)] ($ (layer1 tow_truck_concept3.north) - (0, 0.2) $) -- ( $ (layer2 tow_truck_concept6.south) + (0, 0.25) $);
% \draw[line width=0.44411764705882356mm,-,/pgfplots/color of colormap=(556)] ($ (layer1 tow_truck_concept3.north) - (0, 0.2) $) -- ( $ (layer2 tow_truck_concept5.south) + (0, 0.25) $);
% \draw[line width=0.43888888888888883mm,-,/pgfplots/color of colormap=(562)] ($ (layer3 tow_truck_concept4.north) - (0, 0.2) $) -- ( $ (layer4 tow_truck_concept5.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(295)] ($ (layer3 tow_truck_concept4.north) - (0, 0.2) $) -- ( $ (layer4 tow_truck_concept4.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(491)] ($ (layer3 tow_truck_concept4.north) - (0, 0.2) $) -- ( $ (layer4 tow_truck_concept3.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(267)] ($ (layer3 tow_truck_concept4.north) - (0, 0.2) $) -- ( $ (layer4 tow_truck_concept2.south) + (0, 0.25) $);
% \draw[line width=0.43888888888888883mm,-,/pgfplots/color of colormap=(562)] ($ (layer3 tow_truck_concept1.north) - (0, 0.2) $) -- ( $ (layer4 tow_truck_concept5.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(241)] ($ (layer3 tow_truck_concept1.north) - (0, 0.2) $) -- ( $ (layer4 tow_truck_concept4.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(628)] ($ (layer3 tow_truck_concept1.north) - (0, 0.2) $) -- ( $ (layer4 tow_truck_concept3.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(373)] ($ (layer3 tow_truck_concept1.north) - (0, 0.2) $) -- ( $ (layer4 tow_truck_concept2.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(710)] ($ (layer3 tow_truck_concept1.north) - (0, 0.2) $) -- ( $ (layer4 tow_truck_concept1.south) + (0, 0.25) $);
% \draw[line width=0.5192307692307693mm,-,/pgfplots/color of colormap=(481)] ($ (layer2 tow_truck_concept9.north) - (0, 0.2) $) -- ( $ (layer3 tow_truck_concept4.south) + (0, 0.25) $);
% \draw[line width=0.5863636363636362mm,-,/pgfplots/color of colormap=(414)] ($ (layer2 tow_truck_concept9.north) - (0, 0.2) $) -- ( $ (layer3 tow_truck_concept1.south) + (0, 0.25) $);
% \draw[line width=0.4055555555555556mm,-,/pgfplots/color of colormap=(595)] ($ (layer3 tow_truck_concept5.north) - (0, 0.2) $) -- ( $ (layer4 tow_truck_concept5.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(420)] ($ (layer3 tow_truck_concept5.north) - (0, 0.2) $) -- ( $ (layer4 tow_truck_concept4.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(546)] ($ (layer3 tow_truck_concept5.north) - (0, 0.2) $) -- ( $ (layer4 tow_truck_concept3.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(626)] ($ (layer3 tow_truck_concept5.north) - (0, 0.2) $) -- ( $ (layer4 tow_truck_concept1.south) + (0, 0.25) $);
% \draw[line width=1.0mm,-,/pgfplots/color of colormap=(0)] ($ (layer4 tow_truck_concept5.north) - (0, 0.2) $) -- ( $ (class tow_truck.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(0)] ($ (layer4 tow_truck_concept4.north) - (0, 0.2) $) -- ( $ (class tow_truck.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(0)] ($ (layer4 tow_truck_concept3.north) - (0, 0.2) $) -- ( $ (class tow_truck.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(0)] ($ (layer4 tow_truck_concept1.north) - (0, 0.2) $) -- ( $ (class tow_truck.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(0)] ($ (layer4 tow_truck_concept2.north) - (0, 0.2) $) -- ( $ (class tow_truck.south) + (0, 0.25) $);
\end{scope}
    \end{tikzpicture}
\hspace{0.075cm}
%  \begin{tikzpicture}[
%         every node/.style = {inner sep=0pt},
% every label/.append style = {label distance=2pt, align = center},
%          sibling distance = 4.75em,
%            level 1/.style = {level distance=6em,anchor=north},
%            level 2/.style = {level distance=5.5em,anchor=north},
%            level 3/.style = {level distance=5em,anchor=north},
%            ]  
% \node[anchor=south, label=GoogLeNet](class teapot)
% % \node[anchor=south, label=A Visual Concept Connectome]
% % class teapot
% {\includegraphics[width=25mm]{images/connectomes/googlenet_teapot/class teapot.png}}
%     child {node[](inception5b teapot_concept5){\includegraphics[width=16mm]{images/connectomes/googlenet_teapot/inception5b teapot_concept5.png}} 
%         edge from parent[draw=none]} 
%     child {node[](inception5b teapot_concept4){\includegraphics[width=16mm]{images/connectomes/googlenet_teapot/inception5b teapot_concept4.png}} 
%         edge from parent[draw=none]} 
%     child {node[](inception5b teapot_concept3){\includegraphics[width=16mm]{images/connectomes/googlenet_teapot/inception5b teapot_concept3.png}} 
%         edge from parent[draw=none]
%         child {node[xshift=-0.84cm](inception4c teapot_concept5){\includegraphics[width=16mm]{images/connectomes/googlenet_teapot/inception4c teapot_concept5.png}} 
%             edge from parent[draw=none]}
%         child {node[xshift=-0.84cm](inception4c teapot_concept3){\includegraphics[width=16mm]{images/connectomes/googlenet_teapot/inception4c teapot_concept3.png}} 
%             edge from parent[draw=none]} 
%         child {node[xshift=-0.84cm](inception4c teapot_concept2) {\includegraphics[width=16mm]{images/connectomes/googlenet_teapot/inception4c teapot_concept2.png}}}
%         child {node[xshift=-0.84cm](inception4c teapot_concept1){\includegraphics[width=16mm]{images/connectomes/googlenet_teapot/inception4c teapot_concept1.png}} 
%             edge from parent[draw=none]} 
%             } 
%     child {node[](inception5b teapot_concept2){\includegraphics[width=16mm]{images/connectomes/googlenet_teapot/inception5b teapot_concept2.png}} edge from parent[draw=none]};
% % ARROWS
% \draw[line width=0.7899999999999998mm,-,/pgfplots/color of colormap=(211)] (inception4c teapot_concept5.north) -- (inception5b teapot_concept5.south);
% \draw[line width=0.615mm,-,/pgfplots/color of colormap=(385)] (inception4c teapot_concept5.north) -- (inception5b teapot_concept4.south);
% \draw[line width=0.8833333333333334mm,-,/pgfplots/color of colormap=(117)] (inception4c teapot_concept5.north) -- (inception5b teapot_concept3.south);
% \draw[line width=0.8136363636363633mm,-,/pgfplots/color of colormap=(187)] (inception4c teapot_concept5.north) -- (inception5b teapot_concept2.south);
% \draw[line width=0.675mm,-,/pgfplots/color of colormap=(325)] (inception4c teapot_concept3.north) -- (inception5b teapot_concept5.south);
% \draw[line width=0.695mm,-,/pgfplots/color of colormap=(305)] (inception4c teapot_concept3.north) -- (inception5b teapot_concept4.south);
% \draw[line width=0.7944444444444446mm,-,/pgfplots/color of colormap=(206)] (inception4c teapot_concept3.north) -- (inception5b teapot_concept3.south);
% \draw[line width=0.7499999999999999mm,-,/pgfplots/color of colormap=(251)] (inception4c teapot_concept3.north) -- (inception5b teapot_concept2.south);
% \draw[line width=0.7450000000000001mm,-,/pgfplots/color of colormap=(255)] (inception4c teapot_concept2.north) -- (inception5b teapot_concept4.south);
% \draw[line width=0.8772727272727272mm,-,/pgfplots/color of colormap=(123)] (inception4c teapot_concept2.north) -- (inception5b teapot_concept2.south);
% \draw[line width=1.0mm,-,/pgfplots/color of colormap=(0)] (inception5b teapot_concept5.north) -- (class teapot.south);
% \draw[line width=1.0mm,-,/pgfplots/color of colormap=(0)] (inception5b teapot_concept4.north) -- (class teapot.south);
% \draw[line width=1.0mm,-,/pgfplots/color of colormap=(0)] (inception5b teapot_concept3.north) -- (class teapot.south);
% \draw[line width=1.0mm,-,/pgfplots/color of colormap=(0)] (inception5b teapot_concept2.north) -- (class teapot.south);
% \draw[line width=0.43mm,-,/pgfplots/color of colormap=(570)] (inception4c teapot_concept1.north) -- (inception5b teapot_concept5.south);
% \draw[line width=0.635mm,-,/pgfplots/color of colormap=(365)] (inception4c teapot_concept1.north) -- (inception5b teapot_concept4.south);
% \draw[line width=0.8318181818181817mm,-,/pgfplots/color of colormap=(169)] (inception4c teapot_concept1.north) -- (inception5b teapot_concept2.south);
%     \end{tikzpicture}
%     \hspace{0.15cm}
%     \begin{tikzpicture}[
%         every node/.style = {inner sep=0pt},
% every label/.append style = {label distance=2pt, align = center},
%          sibling distance = 4.75em,
%            level 1/.style = {level distance=6em,anchor=north},
%            level 2/.style = {level distance=5.5em,anchor=north},
%            level 3/.style = {level distance=5em,anchor=north},
%            ]  
% \node[anchor=south, label=MViT](class teapot)
% % \node[anchor=south, label=A Visual Concept Connectome]
% % class teapot
% {\includegraphics[width=25mm]{images/connectomes/mvit_teapot/class teapot.png}}
%     child {node[](15 teapot_concept5){\includegraphics[width=16mm]{images/connectomes/mvit_teapot/15 teapot_concept5.png}} 
%         edge from parent[draw=none]} 
%     child {node[](15 teapot_concept3){\includegraphics[width=16mm]{images/connectomes/mvit_teapot/15 teapot_concept3.png}} 
%         edge from parent[draw=none]} 
%     child {node[](15 teapot_concept4){\includegraphics[width=16mm]{images/connectomes/mvit_teapot/15 teapot_concept4.png}} 
%         edge from parent[draw=none]
%         child {node[xshift=-0.84cm](9 teapot_concept6){\includegraphics[width=16mm]{images/connectomes/mvit_teapot/9 teapot_concept6.png}} 
%             edge from parent[draw=none]}
%         child {node[xshift=-0.84cm](9 teapot_concept2){\includegraphics[width=16mm]{images/connectomes/mvit_teapot/9 teapot_concept2.png}} 
%             edge from parent[draw=none]} 
%         child {node[xshift=-0.84cm](9 teapot_concept1) {\includegraphics[width=16mm]{images/connectomes/mvit_teapot/9 teapot_concept1.png}}}
%         child {node[xshift=-0.84cm](9 teapot_concept3){\includegraphics[width=16mm]{images/connectomes/mvit_teapot/9 teapot_concept3.png}} 
%             edge from parent[draw=none]} 
%             } 
%     child {node[](15 teapot_concept1){\includegraphics[width=16mm]{images/connectomes/mvit_teapot/15 teapot_concept1.png}} edge from parent[draw=none]};
% % ARROWS
% % \draw[line width=0.5709677419354839mm,-,/pgfplots/color of colormap=(430)] (1 teapot_concept2.north) -- (3 teapot_concept1.south);
% % \draw[line width=0.5258064516129033mm,-,/pgfplots/color of colormap=(475)] (1 teapot_concept2.north) -- (3 teapot_concept4.south);
% % \draw[line width=0.36578947368421044mm,-,/pgfplots/color of colormap=(635)] (3 teapot_concept1.north) -- (9 teapot_concept6.south);
% % \draw[line width=0.33055555555555555mm,-,/pgfplots/color of colormap=(670)] (3 teapot_concept1.north) -- (9 teapot_concept1.south);
% % \draw[line width=0.43800000000000006mm,-,/pgfplots/color of colormap=(562)] (3 teapot_concept4.north) -- (9 teapot_concept3.south);
% % \draw[line width=0.3552631578947368mm,-,/pgfplots/color of colormap=(645)] (3 teapot_concept4.north) -- (9 teapot_concept6.south);
% % \draw[line width=0.5125mm,-,/pgfplots/color of colormap=(488)] (3 teapot_concept4.north) -- (9 teapot_concept2.south);
% % \draw[line width=0.3388888888888889mm,-,/pgfplots/color of colormap=(662)] (3 teapot_concept4.north) -- (9 teapot_concept1.south);
% % \draw[line width=0.5483870967741936mm,-,/pgfplots/color of colormap=(452)] (1 teapot_concept1.north) -- (3 teapot_concept1.south);
% % \draw[line width=0.5258064516129032mm,-,/pgfplots/color of colormap=(475)] (1 teapot_concept1.north) -- (3 teapot_concept4.south);
% % \draw[line width=0.3789473684210526mm,-,/pgfplots/color of colormap=(622)] (3 teapot_concept2.north) -- (9 teapot_concept6.south);
% % \draw[line width=0.546875mm,-,/pgfplots/color of colormap=(454)] (3 teapot_concept2.north) -- (9 teapot_concept2.south);
% % \draw[line width=0.3527777777777778mm,-,/pgfplots/color of colormap=(648)] (3 teapot_concept2.north) -- (9 teapot_concept1.south);
% \draw[line width=0.6999999999999998mm,-,/pgfplots/color of colormap=(301)] (9 teapot_concept6.north) -- (15 teapot_concept5.south);
% \draw[line width=0.7250000000000001mm,-,/pgfplots/color of colormap=(275)] (9 teapot_concept6.north) -- (15 teapot_concept3.south);
% \draw[line width=0.8142857142857143mm,-,/pgfplots/color of colormap=(186)] (9 teapot_concept6.north) -- (15 teapot_concept4.south);
% \draw[line width=0.6857142857142856mm,-,/pgfplots/color of colormap=(315)] (9 teapot_concept2.north) -- (15 teapot_concept5.south);
% \draw[line width=0.6583333333333334mm,-,/pgfplots/color of colormap=(342)] (9 teapot_concept2.north) -- (15 teapot_concept1.south);
% \draw[line width=0.6928571428571426mm,-,/pgfplots/color of colormap=(308)] (9 teapot_concept1.north) -- (15 teapot_concept5.south);
% \draw[line width=0.725mm,-,/pgfplots/color of colormap=(275)] (9 teapot_concept1.north) -- (15 teapot_concept3.south);
% \draw[line width=0.7357142857142858mm,-,/pgfplots/color of colormap=(265)] (9 teapot_concept1.north) -- (15 teapot_concept4.south);
% \draw[line width=0.6785714285714284mm,-,/pgfplots/color of colormap=(322)] (9 teapot_concept3.north) -- (15 teapot_concept5.south);
% \draw[line width=0.5750000000000001mm,-,/pgfplots/color of colormap=(425)] (9 teapot_concept3.north) -- (15 teapot_concept3.south);
% % \draw[line width=0.36578947368421044mm,-,/pgfplots/color of colormap=(635)] (3 teapot_concept3.north) -- (9 teapot_concept6.south);
% % \draw[line width=0.44375mm,-,/pgfplots/color of colormap=(557)] (3 teapot_concept3.north) -- (9 teapot_concept2.south);
% % \draw[line width=0.37500000000000006mm,-,/pgfplots/color of colormap=(625)] (3 teapot_concept3.north) -- (9 teapot_concept1.south);
% \draw[line width=1.0mm,-,/pgfplots/color of colormap=(0)] (15 teapot_concept5.north) -- (class teapot.south);
% \draw[line width=1.0mm,-,/pgfplots/color of colormap=(0)] (15 teapot_concept3.north) -- (class teapot.south);
% \draw[line width=0.903061224489796mm,-,/pgfplots/color of colormap=(97)] (15 teapot_concept4.north) -- (class teapot.south);
% \draw[line width=1.0mm,-,/pgfplots/color of colormap=(0)] (15 teapot_concept1.north) -- (class teapot.south);
%     \end{tikzpicture}
%     \hspace{0.15cm}
\vrulesep
\hspace{0.075cm}
    \begin{tikzpicture}[
        every node/.style = {inner sep=0pt},
every label/.append style = {label distance=2pt, align = center},
         sibling distance = 4.75em,
           level 1/.style = {level distance=6em,anchor=north},
           level 2/.style = {level distance=5.5em,anchor=north},
           level 3/.style = {level distance=5em,anchor=north},
           ]  
\node[anchor=south, label=MViT](class tow_truck)
% \node[anchor=south, label=A Visual Concept Connectome]
% class teapot
{\includegraphics[width=25mm]{images/connectomes/new/mvit_tow_truck/class tow_truck.png}}
    child {node[](15 tow_truck_concept1){\includegraphics[width=16mm]{images/connectomes/new/mvit_tow_truck/15 tow_truck_concept1.png}} 
        edge from parent[draw=none]
        child {node[xshift=0.84cm](9 tow_truck_concept3){\includegraphics[width=16mm]{images/connectomes/new/mvit_tow_truck/9 tow_truck_concept3.png}} 
            edge from parent[draw=none]}
        child {node[xshift=0.84cm](9 tow_truck_concept5){\includegraphics[width=16mm]{images/connectomes/new/mvit_tow_truck/9 tow_truck_concept5.png}} 
            edge from parent[draw=none]} 
        child {node[xshift=0.84cm](9 tow_truck_concept2) {\includegraphics[width=16mm]{images/connectomes/new/mvit_tow_truck/9 tow_truck_concept2.png}}
        edge from parent[draw=none]}
            } 
    child {node[](15 tow_truck_concept2){\includegraphics[width=16mm]{images/connectomes/new/mvit_tow_truck/15 tow_truck_concept2.png}} 
    edge from parent[draw=none]};
% ARROWS
\begin{scope}[on background layer]
% \draw[line width=0.6266666666666666mm,-,/pgfplots/color of colormap=(374)] ($ (1 tow_truck_concept10.north) - (0, 0.2) $) -- ( $ (3 tow_truck_concept8.south) + (0, 0.25) $);
% \draw[line width=0.5676470588235294mm,-,/pgfplots/color of colormap=(433)] ($ (1 tow_truck_concept10.north) - (0, 0.2) $) -- ( $ (3 tow_truck_concept5.south) + (0, 0.25) $);
% \draw[line width=0.5842105263157895mm,-,/pgfplots/color of colormap=(416)] ($ (1 tow_truck_concept10.north) - (0, 0.2) $) -- ( $ (3 tow_truck_concept6.south) + (0, 0.25) $);
% \draw[line width=0.4mm,-,/pgfplots/color of colormap=(600)] ($ (3 tow_truck_concept8.north) - (0, 0.2) $) -- ( $ (9 tow_truck_concept3.south) + (0, 0.25) $);
% \draw[line width=0.3717391304347827mm,-,/pgfplots/color of colormap=(629)] ($ (3 tow_truck_concept8.north) - (0, 0.2) $) -- ( $ (9 tow_truck_concept2.south) + (0, 0.25) $);
% \draw[line width=0.4261904761904763mm,-,/pgfplots/color of colormap=(574)] ($ (3 tow_truck_concept8.north) - (0, 0.2) $) -- ( $ (9 tow_truck_concept5.south) + (0, 0.25) $);
% \draw[line width=0.3970588235294117mm,-,/pgfplots/color of colormap=(603)] ($ (3 tow_truck_concept5.north) - (0, 0.2) $) -- ( $ (9 tow_truck_concept3.south) + (0, 0.25) $);
% \draw[line width=0.391304347826087mm,-,/pgfplots/color of colormap=(609)] ($ (3 tow_truck_concept5.north) - (0, 0.2) $) -- ( $ (9 tow_truck_concept2.south) + (0, 0.25) $);
% \draw[line width=0.3428571428571428mm,-,/pgfplots/color of colormap=(658)] ($ (3 tow_truck_concept5.north) - (0, 0.2) $) -- ( $ (9 tow_truck_concept5.south) + (0, 0.25) $);
% \draw[line width=0.5499999999999999mm,-,/pgfplots/color of colormap=(451)] ($ (3 tow_truck_concept6.north) - (0, 0.2) $) -- ( $ (9 tow_truck_concept1.south) + (0, 0.25) $);
% \draw[line width=0.44117647058823534mm,-,/pgfplots/color of colormap=(559)] ($ (3 tow_truck_concept6.north) - (0, 0.2) $) -- ( $ (9 tow_truck_concept3.south) + (0, 0.25) $);
% \draw[line width=0.4195652173913043mm,-,/pgfplots/color of colormap=(581)] ($ (3 tow_truck_concept6.north) - (0, 0.2) $) -- ( $ (9 tow_truck_concept2.south) + (0, 0.25) $);
% \draw[line width=0.4261904761904762mm,-,/pgfplots/color of colormap=(574)] ($ (3 tow_truck_concept6.north) - (0, 0.2) $) -- ( $ (9 tow_truck_concept5.south) + (0, 0.25) $);
% \draw[line width=0.5636363636363637mm,-,/pgfplots/color of colormap=(437)] ($ (1 tow_truck_concept7.north) - (0, 0.2) $) -- ( $ (3 tow_truck_concept1.south) + (0, 0.25) $);
% \draw[line width=0.6366666666666665mm,-,/pgfplots/color of colormap=(364)] ($ (1 tow_truck_concept7.north) - (0, 0.2) $) -- ( $ (3 tow_truck_concept8.south) + (0, 0.25) $);
% \draw[line width=0.5578947368421053mm,-,/pgfplots/color of colormap=(443)] ($ (1 tow_truck_concept7.north) - (0, 0.2) $) -- ( $ (3 tow_truck_concept6.south) + (0, 0.25) $);
% \draw[line width=0.43478260869565216mm,-,/pgfplots/color of colormap=(566)] ($ (3 tow_truck_concept1.north) - (0, 0.2) $) -- ( $ (9 tow_truck_concept2.south) + (0, 0.25) $);
% \draw[line width=0.4428571428571429mm,-,/pgfplots/color of colormap=(558)] ($ (3 tow_truck_concept1.north) - (0, 0.2) $) -- ( $ (9 tow_truck_concept5.south) + (0, 0.25) $);
% \draw[line width=0.5558823529411764mm,-,/pgfplots/color of colormap=(445)] ($ (1 tow_truck_concept3.north) - (0, 0.2) $) -- ( $ (3 tow_truck_concept5.south) + (0, 0.25) $);
% \draw[line width=0.536842105263158mm,-,/pgfplots/color of colormap=(464)] ($ (1 tow_truck_concept3.north) - (0, 0.2) $) -- ( $ (3 tow_truck_concept6.south) + (0, 0.25) $);
% \draw[line width=0.6466666666666665mm,-,/pgfplots/color of colormap=(354)] ($ (1 tow_truck_concept2.north) - (0, 0.2) $) -- ( $ (3 tow_truck_concept8.south) + (0, 0.25) $);
% \draw[line width=0.5270833333333333mm,-,/pgfplots/color of colormap=(473)] ($ (1 tow_truck_concept2.north) - (0, 0.2) $) -- ( $ (3 tow_truck_concept11.south) + (0, 0.25) $);
% \draw[line width=0.5617647058823528mm,-,/pgfplots/color of colormap=(439)] ($ (1 tow_truck_concept2.north) - (0, 0.2) $) -- ( $ (3 tow_truck_concept5.south) + (0, 0.25) $);
% \draw[line width=0.536842105263158mm,-,/pgfplots/color of colormap=(464)] ($ (1 tow_truck_concept2.north) - (0, 0.2) $) -- ( $ (3 tow_truck_concept6.south) + (0, 0.25) $);
% \draw[line width=0.45294117647058824mm,-,/pgfplots/color of colormap=(548)] ($ (3 tow_truck_concept11.north) - (0, 0.2) $) -- ( $ (9 tow_truck_concept3.south) + (0, 0.25) $);
% \draw[line width=0.42391304347826086mm,-,/pgfplots/color of colormap=(577)] ($ (3 tow_truck_concept11.north) - (0, 0.2) $) -- ( $ (9 tow_truck_concept2.south) + (0, 0.25) $);
% \draw[line width=0.3833333333333334mm,-,/pgfplots/color of colormap=(617)] ($ (3 tow_truck_concept11.north) - (0, 0.2) $) -- ( $ (9 tow_truck_concept5.south) + (0, 0.25) $);
% \draw[line width=0.6299999999999998mm,-,/pgfplots/color of colormap=(371)] ($ (1 tow_truck_concept8.north) - (0, 0.2) $) -- ( $ (3 tow_truck_concept8.south) + (0, 0.25) $);
% \draw[line width=0.588235294117647mm,-,/pgfplots/color of colormap=(412)] ($ (1 tow_truck_concept8.north) - (0, 0.2) $) -- ( $ (3 tow_truck_concept5.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(514)] ($ (9 tow_truck_concept2.north) - (0, 0.2) $) -- ( $ (15 tow_truck_concept1.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(419)] ($ (9 tow_truck_concept5.north) - (0, 0.2) $) -- ( $ (15 tow_truck_concept2.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(432)] ($ (9 tow_truck_concept3.north) - (0, 0.2) $) -- ( $ (15 tow_truck_concept2.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(0)] ($ (15 tow_truck_concept2.north) - (0, 0.2) $) -- ( $ (class tow_truck.south) + (0, 0.25) $);
\draw[line width=0.6mm,-,/pgfplots/color of colormap=(737)] ($ (15 tow_truck_concept1.north) - (0, 0.2) $) -- ( $ (class tow_truck.south) + (0, 0.25) $);
\end{scope}
    \end{tikzpicture}
}\vspace{-0.3cm}
\caption{\textcolor{blue}{VCCs for a ConvNet (ResNet50) and transformer (MViT) for the class `Tow Truck'. Shown are only the last two layers with the class output.}
%Similarly to Fig.~\ref{fig:cnn_trans}, ViT-b has more diversity in the connections between concepts at the later layers of the model compared to ResNet50. At all observed layers, ConvNets appear to attend more to the background scene than the transformers. 
% \textcolor{red}{Caption says 3 layers, as does implementation details, but figure only shows 3.}
}
\label{fig:cnn_trans_vcc_compare} \vspace{-0.4cm}
\end{figure}


%\subsubsection{Inter-layer concept weight validation} \label{sec:validateITCAV}
\textbf{ITCAV validation.} If the interlayer concept connection weights are meaningful, then the accumulated weights from earlier to later layer concepts should be correlated with their probability of predicting the target class.
%impact on final classification. 
We use this intuition to validate our ITCAV approach to recovering interlayer concept weights as follows. 
%We now validate the efficacy of the ITCAV method for estimating connection strength between concepts at different layers. First, 
We define the average path strength (APS), a scalar value between zero and one representing the average strength of the connection between a concept and the class logit. Given concept $\textbf{q}_j$ at layer $j$, let there be $L$ layers in the VCC between the concept and the logit layer; thus, each path from the concept to the logit consists of $L$ edge weights. We consider all possible paths in the VCC from this concept to the class logit. Let $e_{\textbf{q}_j}(l,p)$ be the edge weight (\ie ITCAV score) of the $p^{\text{th}}$ path (from concept $\textbf{q}_j$ to the class concept) for VCC layer $l$. To calculate the APS score for a given concept, we average over all paths, $P$, and edge weights in each path to get
\begin{equation}\label{eq:APS}
    \text{APS}(\textbf{q}_j) = \frac{1}{P}\sum_{p=1}^P \big[\frac{1}{L}\sum_{l=1}^L e_{\textbf{q}_j}(l,p)\big].
\end{equation}
% where $\text{APS}(\textbf{q})$ represents the strength of the connection (\ie positive contribution) between concept $\textbf{q}_l^i$ and the class logit based on the ITCAV edge weights. 
%One would expect that a model classifying segments belonging to a concept with a large APS score would have a higher probability of predicting the target class, and a lower probability when classifying segments belonging to a concept with a small APS score.
% One would expect that segments belonging to a concept with a large APS score would have a positive contribution to the probability of observing the target class, while segments belonging to a concept with a small APS score would have a small contribution. 
%Following this line of intuition, 
Next, we calculate the logit sum (LS) score for a given concept, $\textbf{q}_j$, by passing all of the corresponding masked segments, $\mathbf{M}_{\textbf{q}_j}$, through the model, $F(\cdot)$. We then sum up the logit scores for the target class, $c$, to yield
\vspace{-4pt}
\begin{equation}\label{eq:ssc}
    \text{LS}(\textbf{q}_j) = \sum_{i=1}^{|\mathbf{M}_{\textbf{q}_j}|} F(\mathbf{M}^i_{\textbf{q}_j})|_c,
\end{equation}
where $\mathbf{M}^i_{\textbf{q}_j}$ denotes the $i^{\text{th}}$ segment mask, and $F(\cdot)|_c$ denotes the $c^{\text{th}}$ logit score. If the ITCAV edge weights are meaningful, then there should be positive correlation between the APS and LS scores, \ie $ \text{APS(\textbf{q})} \propto \text{LS(\textbf{q})}$.

























Figure~\ref{fig:ITCAV_validation} shows the LS scores plotted against the APS scores for 
ResNet50~\cite{he2016deep}, GoogLeNet~\cite{szegedy2015going}, MViT~\cite{fan2021multiscale} and ViT-b~\cite{vaswani2017attention}.
% ResNet18~\cite{he2016deep} (layer names: \textit{layer1}, \textit{layer2}, \textit{layer3}, \textit{layer4}), GoogLeNet~\cite{szegedy2015going} (layer names: \textit{conv3}, \textit{inception3b}, \textit{inception4c}, \textit{inception5b}), and VGG16~\cite{simonyan2014very} (layer names: \textit{8}, \textit{15}, \textit{22}, \textit{29}).
A positive correlation is found between the APS and LS scores for all architectures. Indeed, these results suggest that the combination of ITCAV scores is predictive of whether a concept is representative of the target class. The supplement has additional LS vs.\ APS plots with other models to further support these findings. 






\begin{figure} [t]
	\begin{center}
     \centering 
\resizebox{0.48\textwidth}{!}{
\hspace{0.1cm}
\begin{tikzpicture} 
                 \begin{axis}[
                 line width=1.0,
                 % title={Branching Factor},
                 title style={at={(axis description cs:0.5,1.2)},anchor=north,font=\normalsize},
                 % xlabel={Top-k \% Units Masked},
                 ylabel={Branching Factor},
                 xmin=0, xmax=1,
                 ymin=0, ymax=17,
                 xtick={0,0.2,0.4,0.6,0.8,1},
                %  ytick={30, 35, 40, 45, 50, 55, 60, 65, 70},
                 x tick label style={font=\tiny, rotate=0, anchor=north},
                 y tick label style={font=\tiny},
                 x label style={at={(axis description cs:0.5,0.09)},anchor=north,font=\small},
                 y label style={at={(axis description cs:0.2,.5)},anchor=south,font=\small},
                 width=6.5cm,
                 height=4.0cm, % height=4.3cm, 
                 ymajorgrids=false,
                 xmajorgrids=false,
                 major grid style={dotted,green!20!black},
                 % legend columns=2,
                 % legend style={
                 %  nodes={scale=0.7, transform shape},
                 %  cells={anchor=west},
                 %  legend style={at={(0.5,1)},anchor=north,row sep=0.01pt}, font =\small}
             ]
            % \addlegendentry{VGG16}
            \addplot[dashed,line width=0.9pt, mark size=1.6pt, color=blue, mark=diamond,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(0.31, 6.765)
                                  (0.54, 6.249)
                                  (0.77, 4.599)
                                  (1, 1.696)};
            % \addlegendentry{VGG16}
            \addplot[line width=0.9pt, mark size=1.6pt, color=blue, mark=diamond,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(0.08,12.627)
                                    (0.15,13.484)
                                    (0.23,9.301)
                                    (0.31,16.194)
                                    (0.38,12.628)
                                    (0.46,12.349)
                                    (0.54,12.888)
                                    (0.62,13.575)
                                    (0.69,14.122)
                                    (0.77,9.5)
                                    (0.85,7.28)
                                    (0.92,5.367)
                                    (1.00,2)}; 

                                    
            % \addlegendentry{MobileNet-v3}
            \addplot[dashed,line width=0.9pt, mark size=1.6pt, color=brown, mark=triangle,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(0.06, 7.102)
                                  (0.38, 5.175)
                                  (0.75, 4.3)
                                  (1, 1.149)};  
            \addplot[line width=0.9pt, mark size=1.6pt, color=brown, mark=triangle,error bars/.cd, y dir=both, y explicit,]
                     coordinates {
                                (0.06,10.927)
                                (0.13,9.423)
                                (0.19,10.839)
                                (0.25,12.01)
                                (0.31,14.332)
                                (0.38,12.99)
                                (0.44,10.975)
                                (0.50,8.478)
                                (0.56,8.016)
                                (0.63,6.384)
                                (0.69,7.857)
                                (0.75,6.81)
                                (0.81,4.642)
                                (0.88,2.685)
                                (0.94,3.55)
                                (1.00,0.4)};     
              \end{axis}
\end{tikzpicture}
\hspace{0.1cm}
\begin{tikzpicture} 
                  \begin{axis}[
                 line width=1.0,
                 % title={Concepts},
                 title style={at={(axis description cs:0.5,1.2)},anchor=north,font=\normalsize},
                 % xlabel={Layer},
                 ylabel={Number of Concepts},
                 xmin=0, xmax=1,
                 ymin=1.5, ymax=21,
                 xtick={0,0.2,0.4,0.6,0.8,1},
                %  ytick={30, 35, 40, 45, 50, 55, 60, 65, 70},
                 x tick label style={font=\tiny, rotate=0, anchor=north},
                 y tick label style={font=\tiny},
                 x label style={at={(axis description cs:0.5,0.09)},anchor=north,font=\small},
                 y label style={at={(axis description cs:0.2,.5)},anchor=south,font=\small},
                 width=6.5cm,
                 height=4.0cm, % height=4.3cm, 
                 ymajorgrids=false,
                 xmajorgrids=false,
                 major grid style={dotted,green!20!black},
                 legend columns=2,
                 legend style={
                  nodes={scale=0.7, transform shape},
                  cells={anchor=west},
                  legend style={at={(0.5,1)},anchor=north,row sep=0.01pt}, font =\small}
             ]
            % \addlegendentry{VGG16}
            \addplot[dashed,line width=0.9pt, mark size=1.6pt, color=blue, mark=diamond,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(0.31, 11.174)
                                  (0.54, 9.348)
                                  (0.77, 6.348)
                                  (1, 3.087)};
            \addplot[line width=0.9pt, mark size=1.6pt, color=blue, mark=diamond,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(0.08,17.2)
                                (0.15,18.6)
                                (0.23,20.2)
                                (0.31,20.6)
                                (0.38,19.2)
                                (0.46,16.4)
                                (0.54,14.9)
                                (0.62,13.6)
                                (0.69,14.2)
                                (0.77,9.5)
                                (0.85,7.3)
                                (0.92,5.5)
                                (1.00,3.2)};

                                  
            % \addlegendentry{MobileNet-v2}
            \addplot[dashed,line width=0.9pt, mark size=1.6pt, color=brown, mark=triangle,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(0.06, 12.255)
                                  (0.38, 9.532)
                                  (0.75, 6.936)
                                  (1, 2.404)};
                % \addlegendentry{MobileNet-v2}
            \addplot[line width=0.9pt, mark size=1.6pt, color=brown, mark=triangle,error bars/.cd, y dir=both, y explicit,]
                     coordinates {
                                (0.06,16.1)
                                (0.13,18)
                                (0.19,18.4)
                                (0.25,19.9)
                                (0.31,19.8)
                                (0.38,18.2)
                                (0.44,15)
                                (0.50,11.8)
                                (0.56,10.7)
                                (0.63,11.5)
                                (0.69,9.7)
                                (0.75,9.1)
                                (0.81,6.9)
                                (0.88,6.4)
                                (0.94,3.6)
                                (1.00,2.3)};                               
              \end{axis}
\end{tikzpicture}}
\resizebox{0.48\textwidth}{!}{
\hspace{0.1cm}
% \vspace{-0.2}
\begin{tikzpicture}
                 \begin{axis}[
                 line width=1.0,
                 % title={Branching Factor},
                 title style={at={(axis description cs:0.5,1.2)},anchor=north,font=\normalsize},
                 xlabel={Layer},
                 ylabel={Edge Weight Average},
                 xmin=0, xmax=1,
                 ymin=0, ymax=1.2,
                 xtick={0,0.2,0.4,0.6,0.8,1},
                %  ytick={30, 35, 40, 45, 50, 55, 60, 65, 70},
                 x tick label style={font=\tiny, rotate=0, anchor=north},
                 y tick label style={font=\tiny},
                 x label style={at={(axis description cs:0.5,0.15)},anchor=north,font=\small},
                 y label style={at={(axis description cs:0.2,.5)},anchor=south,font=\small},
                 width=6.5cm,
                 height=4.0cm, % height=4.3cm, 
                 ymajorgrids=false,
                 xmajorgrids=false,
                 major grid style={dotted,green!20!black},
                 legend columns=2,
                 legend style={
                  nodes={scale=0.6, transform shape},
                  cells={anchor=west},
                  legend style={at={(0.5,1)},anchor=north,row sep=0.01pt}, font =\small}
             ]

            \addlegendentry{4-VGG16}
            \addplot[dashed,line width=0.9pt, mark size=1.6pt, color=blue, mark=diamond,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(0.31, 0.329)
                                  (0.54, 0.272)
                                  (0.77, 0.429)
                                  (1.00, 0.801)};
            \addlegendentry{All-VGG16}
            \addplot[line width=0.9pt, mark size=1.6pt, color=blue, mark=diamond,error bars/.cd, y dir=both, y explicit,]
                     coordinates {
                                (0.08,0.566)
                                (0.15,0.659)
                                (0.23,0.607)
                                (0.31,0.609)
                                (0.38,0.568)
                                (0.46,0.391)
                                (0.54,0.334)
                                (0.62,0.214)
                                (0.69,0.107)
                                (0.77,0.197)
                                (0.85,0.132)
                                (0.92,0.08)
                                (1.00,0.79)};

            \addlegendentry{4-MobileNet-v3}
            \addplot[dashed,line width=0.9pt, mark size=1.6pt, color=brown, mark=triangle,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(0.06, 0.471)
                                  (0.38, 0.529)
                                  (0.75, 0.395)
                                  (1, 0.755)};  
            \addlegendentry{All-MobileNet-v3}
            \addplot[line width=0.9pt, mark size=1.6pt, color=brown, mark=triangle,error bars/.cd, y dir=both, y explicit,]
                     coordinates {
                                (0.06,0.49)
                                (0.13,0.393)
                                (0.19,0.374)
                                (0.25,0.468)
                                (0.31,0.375)
                                (0.38,0.38)
                                (0.44,0.341)
                                (0.50,0.357)
                                (0.56,0.407)
                                (0.63,0.55)
                                (0.69,0.417)
                                (0.75,0.56)
                                (0.81,0.392)
                                (0.88,0.455)
                                (0.94,0.114)
                                (1.00,0.629)};  
              \end{axis}
\end{tikzpicture}
\hspace{0.1cm}
\begin{tikzpicture} 
                  \begin{axis}[
                 line width=1.0,
                 % title={Branching Factor},
                 title style={at={(axis description cs:0.5,1.2)},anchor=north,font=\normalsize},
                 xlabel={Layer},
                 ylabel={Edge Weight Variance},
                 xmin=0, xmax=1,
                 ymin=0, ymax=0.04,
                 xtick={0,0.2,0.4,0.6,0.8,1},
                %  ytick={30, 35, 40, 45, 50, 55, 60, 65, 70},
                 x tick label style={font=\tiny, rotate=0, anchor=north},
                 y tick label style={font=\tiny},
                 x label style={at={(axis description cs:0.5,0.15)},anchor=north,font=\small},
                 y label style={at={(axis description cs:0.2,.5)},anchor=south,font=\small},
                 width=6.5cm,
                 height=4.0cm, % height=4.3cm, 
                 ymajorgrids=false,
                 xmajorgrids=false,
                 major grid style={dotted,green!20!black},
                    legend columns=2,
                 legend style={
                  nodes={scale=0.7, transform shape},
                  cells={anchor=west},
                  legend style={at={(0.405,1)},anchor=north,row sep=0.01pt}, font =\small}
             ]
            \addplot[dashed,line width=0.9pt, mark size=1.6pt, color=blue, mark=diamond,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(0.31, 0.008)
                                  (0.54, 0.013)
                                  (0.77, 0.007)
                                  (1, 0.003)}; 
            \addplot[line width=0.9pt, mark size=1.6pt, color=blue, mark=diamond,error bars/.cd, y dir=both, y explicit,]
                     coordinates {
                                (0.08,0.034)
                                (0.15,0.03)
                                (0.23,0.031)
                                (0.31,0.024)
                                (0.38,0.019)
                                (0.46,0.009)
                                (0.54,0.007)
                                (0.62,0.005)
                                (0.69,0.003)
                                (0.77,0.004)
                                (0.85,0.004)
                                (0.92,0.003)
                                (1.00,0.003)}; 
                                  
            \addplot[dashed,line width=0.9pt, mark size=1.6pt, color=brown, mark=triangle,error bars/.cd, y dir=both, y explicit,]
                     coordinates {(0.06, 0.008)
                                  (0.38, 0.008)
                                  (0.75, 0.006)
                                  (1.00, 0.004)};
            \addplot[line width=0.9pt, mark size=1.6pt, color=brown, mark=triangle,error bars/.cd, y dir=both, y explicit,]
                     coordinates {
                                (0.06,0.02)
                                (0.13,0.02)
                                (0.19,0.018)
                                (0.25,0.023)
                                (0.31,0.022)
                                (0.38,0.019)
                                (0.44,0.009)
                                (0.50,0.004)
                                (0.56,0.003)
                                (0.63,0.003)
                                (0.69,0.002)
                                (0.75,0.002)
                                (0.81,0.002)
                                (0.88,0.003)
                                (0.94,0.003)
                                (1.00,0.004)};
  
                             
              \end{axis}
\end{tikzpicture}
}
\end{center}
\vspace{-0.6cm}
\caption{Graph metrics comparing all-layer VCCs for MobileNetv3, VGG16 and MViT. 
%The number of concepts varies at early and middle layers but converges to around five concepts in the final layer. The average edge weight and edge variance are also less strong and more diverse, respectively, in the final layers for transformer architectures than for CNNs.
}\label{fig:local_global}
\vspace{-0.5cm}
\end{figure}


% Our second observation is that higher layers tend to have the highest LS and APS scores. This is to be expected, as the features from these layers contain image regions closer to the object. d
% Another interesting observation is that certain concepts can have a negative contribution on the 

\begin{figure*}
   \centering   
\includegraphics[width=0.96\textwidth]{images/figures/Debug2.png}\vspace{-0.3cm}
    \caption{\textcolor{blue}{Debugging model failure modes with VCCs. We show an image of a tricycle incorrectly predicted by a ResNet50 as a rickshaw (middle) as well as the top-down segmentation of the image (Sec.~\ref{sec:divisive_cluster}). We also show the incorrect (left) and correct (right) VCCs. Following the hierarchy of concepts reveals that the model focused heavily on the collapsible hood, starting at Layer 2.}}\label{fig:debug}\vspace{-0.5cm}
\end{figure*}


\subsection{Understanding models with VCCs}\label{sec:architectures}
Figure~\ref{fig:goog_jay} shows a single example of a three layer VCC for the GoogLeNet~\cite{szegedy2015going} model targeting the class ``Jay''. Notice how the inception5b `bird' concepts ($c_{51},c_{52}$) are formed as selective weighting of inception4c concepts background ($c_{41}$), bird part ($c_{42},c_{44}$) and tree branch ($c_{43}$), while the inception5b background concepts ($c_{53},c_{54}$) are differently formed from weighting of solely inception4c background part concepts (\eg tree branch ($c_{43}$) and green leaves ($c_{41}$)). Further, the concepts found in inception4c are composed from varying combinations of colors and parts found in conv3 (\eg. various bird parts ($c_{31},c_{33}$) contribute to the bird concepts at inception4c). In the end, both scene and object contribute with strong weights to the final category.

We now compare VCCs generated for the ConvNet and transformer-based architectures listed in Sec.~\ref{sec:implementation_details}.  We use standard metrics for analyzing tree-like data structures in a per-layer fashion: (1) branching factor (extent to which the representation is distributed), (2) number of nodes (how many concepts the model uses to encode a particular class), (3) edge weights (strength of connection between concepts), and (4) edge weight variance (variability of connection strength). We calculate averages over 50 VCCs for 50 randomly selected ImageNet classes.
%We compute the VCCs for 50 randomly selected ImageNet classes, and take the average over all 50 connectomes. 





%For ConvNets, we consider four standard architectures, ResNet50~\cite{he2016deep}, GoogLeNet~\cite{szegedy2015going}, VGG-16~\cite{simonyan2014very}, and MobileNetv2~\cite{sandler2018mobilenetv2}. For transformers, we consider the standard ViT-b~\cite{vaswani2017attention} and the Multiscale ViT (MViT)~\cite{fan2021multiscale}. 
% \textcolor{pink}{We find that the branching factor and the number of concepts for both architecture types generally follow a similar pattern of increasing from the early to late layers \ie both types learn more distributed representations deeper in their networks. While the number of concepts differs between architectures in the early and middle layers, they converge to approximately five in the final layer. The edge weights show greater differences between architecture types in two ways. (1) Transformers have more diverse connection strengths in the final layers compared to ConvNets.}
\textbf{Four-layer VCC analysis.} \textcolor{blue}{Figure~\ref{fig:cnn_trans} shows the architecture comparisons. We find that the number of concepts and average edge weights value generally follow a similar pattern. There are more concepts at early layers with weaker corresponding edge weights, while fewer concepts and stronger edge weights at the later layers. This is intuitive as multiple classes share similar low-level concepts (\eg edges, colors, textures) while there are fewer concepts relating to the target class, \ie at the final layers, thus resulting in larger ITCAV values. 
Notably, the branching factor for CNNs monotonically decrease while transformers have consistent branching factors until the last layer. Furthermore, while the branching factor is diverse at the early layers, it converges to approximately two by the final layer for all models, indicating that transformers compose concepts out of a constant number of lower concepts (\ie ~3 for ViT and 6 for MViT) until the final layer. Additionally, the variance of the final layer edge weight is larger for transformer architectures than for ConvNets. This suggests that ConvNets distinguish less between earlier layer concepts and rely mainly on the final representation, while the transformers better distinguish the relative importance of earlier concepts as they assemble later concepts, which could be a reason that transformers often provide better classification (\ie all information is not equally valuable).}
% These differences suggest that in the final layer before the model output, transformers learn a combination of concepts that provide negative and positive contributions to the model output, whereas ConvNets learn concepts that mainly contribute positively to the model output. 
% \textcolor{red}{RW: Why does that interpretation hold? I don't see evidence for negative contributions. Can't it rather be that the ConvNets distinguish less between the earlier layer concepts, while the transformers better distinguish the relative importance of earlier concepts as they assemble later concepts, which could, in turn, be a reason that transformers often provide better classification (\ie all information is not equally valuable)?}

Qualitative examples of VCCs generated for a ConvNet and transformer are shown in Fig.~\ref{fig:cnn_trans_vcc_compare}. 
We limit visualization to two (diverse) models and two later layers with class output for space.
\textcolor{blue}{It can be observed that the connection diversity in the last layer is indeed larger for the transformer vs.\ the ConvNet. Notably, over half of the concepts in the ConvNet capture background centric concepts, while the transformer has only a single background centric concept.}
% Further, as observed in Fig.~\ref{fig:cnn_trans}, the transformer intra-concept segments generally are more varied. For example, concept three in the late layer contains both foreground and background segments, while the background concepts in the ConvNet contain no segments that highlight the teapot region. 
% These observations provide further support \textcolor{red}{WHAT? MK: TBD}


% forklift
% r50 looks for background more than clip
% stronger connections in CLIP early layers

% paper towel
% stole




% \begin{table}[t]
%     \centering
%         \resizebox{0.48\textwidth}{!}{
%         \begin{tabu}{c cccccc}
%         \tabucline[1pt]{-}
%              & \multicolumn{2}{c}{\textbf{Branching Factor}}  & \multicolumn{2}{c}{\textbf{Number of Concepts}} & \multicolumn{2}{c}{\textbf{Edge Weight Ave.}}\\
%              \hline
%               & R50 & CLIP & R50 & CLIP & R50 &  CLIP \\
%              \tabucline[1pt]{-}
%              Layer1 & 5.484 & 6.824 & 10.447 & 11.085 & 0.414 & 0.417\\ 
%              Layer2 & 4.945 & 4.141 & 8.000  & 7.468   & 0.554 & 0.54 \\ 
%              Layer3 & 2.799 & 2.754 & 5.106  & 5.702  & 0.476 & 0.563\\ 
%              Layer4 & 2.915 & 1.574 & 2.957  & 2.383  & 0.917 & 0.634\\ 
%              \hline
%              Variance & $\pm$ 1.90 & $\pm$ 5.10 & $\pm$ 10.75 & $\pm$ 13.15 & $\pm$ 0.05 & $\pm$ 0.01 \\
%         \tabucline[1pt]{-}
%         \end{tabu}}
% \vspace{-8pt}
%     \caption{VCC metrics for ResNet50~\cite{he2016deep} trained on ImageNet~\cite{deng2009imagenet} and via contrastive image-language pretraining (CLIP)~\cite{radford2021learning}. \textcolor{red}{For all metrics, the CLIP-trained model has comparatively less variance across layers.}}
%     \label{tab:clip_r50_compare}
%     \vspace{-12pt}
% \end{table}


% \subsection{Understanding tasks with VCCs
% %Object Recognition vs. Image-Language Contrastive Learning
% }\label{sec:tasks}

% We now explore how VCCs can reveal the effect of the training task on learned concepts and their connections. In particular, given the recent advances of image-language training paradigms, we  compare the standard ResNet50~\cite{he2016deep} model trained on ImageNet~\cite{deng2009imagenet} with ResNet50 trained via Contrastive Language Image Pretraining (CLIP)~\cite{radford2021learning}.

% %ResNet50 model against the standard ResNet50~\cite{he2016deep} model trained on ImageNet~\cite{deng2009imagenet}. The CLIP model is composed of an image encoder and a textual encoder. It is trained on a web-scraped dataset of approximately 400 million image-caption pairs~\cite{radford2021learning} and is optimized to minimize the cosine distance between the embeddings of corresponding image and caption pairs. 



% Table~\ref{tab:clip_r50_compare} compares graph metrics over VCC layers between the two models at four residual blocks. 
% \textcolor{red}{We find that CLIP-ResNet50 has on average 0.88 more concepts in the first two layers than ImageNet-ResNet50. Also, the average edge weight for \textit{Layer2} is 0.17 larger for CLIP-ResNet50. Further, the variance of all three metrics \textit{across} the layers is much lower for  CLIP-ResNet50. Together, these findings suggest that CLIP-based training guides ResNet50 to learn more concepts with stronger connections at the early layers compared to traditional ImageNet training.} 

% Figure~\ref{fig:clip_r50_vcc_compare} compares VCCs for ImageNet-ResNet50 and CLIP-ResNet50 for the class `Forklift'. For the ImageNet trained model, the majority of strong connections between concepts are in the last two layers (\ie between \textit{Layer3} and \textit{Layer4}, and between \textit{Layer4} and the class logit). In contrast, all layers in the CLIP trained model contain a diverse range of connection strengths, with more sparsity between \textit{Layer3} and \textit{Layer4}, in particular. Looking at the concept segments themselves reveals additional interesting properties. For example, in the ImageNet trained model, both background and foreground concepts have large connection weights to the class concept, while in the CLIP trained model, the background concepts have weak contributions to the class concept. This further supports the previous finding in Sec.~\ref{sec:architectures} that found ImageNet trained ConvNets rely heavily on background concepts in the later model layers.

% % \textcolor{red}{It seems that the last paragraph suggests more diverse connections across layers, while previous one suggested more uniformity. Need to resolve apparent inconsistency. MK: Will do.}

% %These observations further support \textcolor{red}{WHAT?}








% \begin{figure}[t]
%     \centering
%     \resizebox{0.48\textwidth}{!}{    
%     \begin{tikzpicture}[grow=left,
%         every node/.style = {inner sep=0pt},
% every label/.append style = {label distance=0.5pt, align = center},
%          sibling distance = 5.0em,
%            level 1/.style = {level distance=5em,anchor=east},
%            level 2/.style = {level distance=5em,anchor=east},
%            level 3/.style = {level distance=5em,anchor=east},
%            level 4/.style = {level distance=5em,anchor=east},
%            level 5/.style = {level distance=5em,anchor=east},
%            ]  
% \node[anchor=south,label=Forklift](class forklift)
% {\includegraphics[width=25mm]{images/connectomes/r50_forklift/class forklift.png}}
%     child {node[label={[yshift=-0.08cm]Layer4}](layer4 forklift_concept7){\includegraphics[width=17mm]{images/connectomes/r50_forklift/layer4 forklift_concept7.png}} 
%         edge from parent[draw=none]} 
%     child {node[](layer4 forklift_concept6){\includegraphics[width=17mm]{images/connectomes/r50_forklift/layer4 forklift_concept6.png}} 
%         edge from parent[draw=none]} 
%     child {node[](layer4 forklift_concept5){\includegraphics[width=17mm]{images/connectomes/r50_forklift/layer4 forklift_concept5.png}} 
%         edge from parent[draw=none]
%         child {node[label={[yshift=-0.08cm]Layer3}](layer3 forklift_concept5){\includegraphics[width=17mm]{images/connectomes/r50_forklift/layer3 forklift_concept5.png}} 
%             edge from parent[draw=none]}
%         child {node[](layer3 forklift_concept2){\includegraphics[width=17mm]{images/connectomes/r50_forklift/layer3 forklift_concept2.png}} 
%             edge from parent[draw=none]} 
%         child {node[](layer3 forklift_concept4) {\includegraphics[width=17mm]{images/connectomes/r50_forklift/layer3 forklift_concept4.png}} 
%             edge from parent[draw=none]
%             child {node[label={[yshift=-0.08cm]Layer2}](layer2 forklift_concept3){\includegraphics[width=17mm]{images/connectomes/r50_forklift/layer2 forklift_concept3.png}} 
%             edge from parent[draw=none]}
%             child {node[](layer2 forklift_concept2){\includegraphics[width=17mm]{images/connectomes/r50_forklift/layer2 forklift_concept2.png}} 
%             edge from parent[draw=none]
%                 child {node[label={[yshift=-0.08cm]Layer1}](layer1 forklift_concept1){\includegraphics[width=17mm]{images/connectomes/r50_forklift/layer1 forklift_concept1.png}} 
%                 edge from parent[draw=none]}
%                 child {node[](layer1 forklift_concept2){\includegraphics[width=17mm]{images/connectomes/r50_forklift/layer1 forklift_concept2.png}} 
%                 edge from parent[draw=none]}
%             }
%             child {node[](layer2 forklift_concept1){\includegraphics[width=17mm]{images/connectomes/r50_forklift/layer2 forklift_concept1.png}} 
%             edge from parent[draw=none]}
%             }
%         child {node[](layer3 forklift_concept3){\includegraphics[width=17mm]{images/connectomes/r50_forklift/layer3 forklift_concept3.png}} 
%             edge from parent[draw=none]} 
%         child {node[](layer3 forklift_concept1){\includegraphics[width=17mm]{images/connectomes/r50_forklift/layer3 forklift_concept1.png}} 
%             edge from parent[draw=none]}
%             } 
%     child {node[](layer4 forklift_concept4){\includegraphics[width=17mm]{images/connectomes/r50_forklift/layer4 forklift_concept4.png}} edge from parent[draw=none]
%             }
%     child {node[](layer4 forklift_concept3){\includegraphics[width=17mm]{images/connectomes/r50_forklift/layer4 forklift_concept3.png}} edge from parent[draw=none]
%             };
% % ARROWS
% \begin{scope}[on background layer]
% % \draw[line width=0.36486486486486497mm,-,/pgfplots/color of colormap=(636)] (layer1 forklift_concept1.east) -- (layer2 forklift_concept3.west);
% % \draw[line width=0.5115384615384615mm,-,/pgfplots/color of colormap=(489)] (layer1 forklift_concept1.east) -- (layer2 forklift_concept2.west);
% % \draw[line width=0.3653846153846154mm,-,/pgfplots/color of colormap=(635)] (layer2 forklift_concept3.east) -- (layer3 forklift_concept5.west);
% % \draw[line width=0.3863636363636363mm,-,/pgfplots/color of colormap=(614)] (layer2 forklift_concept3.east) -- (layer3 forklift_concept2.west);
% % \draw[line width=0.5153846153846153mm,-,/pgfplots/color of colormap=(485)] (layer2 forklift_concept3.east) -- (layer3 forklift_concept4.west);
% % \draw[line width=0.27352941176470585mm,-,/pgfplots/color of colormap=(727)] (layer2 forklift_concept3.east) -- (layer3 forklift_concept3.west);
% % \draw[line width=0.4000000000000001mm,-,/pgfplots/color of colormap=(600)] (layer2 forklift_concept2.east) -- (layer3 forklift_concept5.west);
% % \draw[line width=0.3961538461538462mm,-,/pgfplots/color of colormap=(604)] (layer2 forklift_concept2.east) -- (layer3 forklift_concept1.west);
% % \draw[line width=0.3022727272727273mm,-,/pgfplots/color of colormap=(698)] (layer2 forklift_concept2.east) -- (layer3 forklift_concept2.west);
% % \draw[line width=0.3117647058823529mm,-,/pgfplots/color of colormap=(689)] (layer2 forklift_concept2.east) -- (layer3 forklift_concept3.west);
% % \draw[line width=0.39729729729729724mm,-,/pgfplots/color of colormap=(603)] (layer1 forklift_concept2.east) -- (layer2 forklift_concept3.west);
% % \draw[line width=0.5480769230769229mm,-,/pgfplots/color of colormap=(452)] (layer1 forklift_concept2.east) -- (layer2 forklift_concept2.west);
% % \draw[line width=0.9100000000000001mm,-,/pgfplots/color of colormap=(90)] (layer3 forklift_concept5.east) -- (layer4 forklift_concept7.west);
% % \draw[line width=0.7166666666666668mm,-,/pgfplots/color of colormap=(284)] (layer3 forklift_concept5.east) -- (layer4 forklift_concept6.west);
% % \draw[line width=0.8650000000000002mm,-,/pgfplots/color of colormap=(135)] (layer3 forklift_concept5.east) -- (layer4 forklift_concept5.west);
% % \draw[line width=0.7857142857142857mm,-,/pgfplots/color of colormap=(215)] (layer3 forklift_concept5.east) -- (layer4 forklift_concept4.west);
% % \draw[line width=0.8111111111111112mm,-,/pgfplots/color of colormap=(189)] (layer3 forklift_concept5.east) -- (layer4 forklift_concept3.west);
% % % \draw[line width=0.85mm,-,/pgfplots/color of colormap=(150)] (layer3 forklift_concept5.east) -- (layer4 forklift_concept2.west);
% % % \draw[line width=0.7499999999999998mm,-,/pgfplots/color of colormap=(251)] (layer3 forklift_concept5.east) -- (layer4 forklift_concept1.west);
% % \draw[line width=0.7500000000000001mm,-,/pgfplots/color of colormap=(250)] (layer3 forklift_concept2.east) -- (layer4 forklift_concept7.west);
% % \draw[line width=0.6333333333333334mm,-,/pgfplots/color of colormap=(367)] (layer3 forklift_concept2.east) -- (layer4 forklift_concept6.west);
% % \draw[line width=0.7649999999999999mm,-,/pgfplots/color of colormap=(236)] (layer3 forklift_concept2.east) -- (layer4 forklift_concept5.west);
% % \draw[line width=0.8500000000000002mm,-,/pgfplots/color of colormap=(150)] (layer3 forklift_concept2.east) -- (layer4 forklift_concept3.west);
% % % \draw[line width=0.8142857142857143mm,-,/pgfplots/color of colormap=(186)] (layer3 forklift_concept2.east) -- (layer4 forklift_concept2.west);
% % \draw[line width=0.7900000000000001mm,-,/pgfplots/color of colormap=(210)] (layer3 forklift_concept4.east) -- (layer4 forklift_concept7.west);
% % \draw[line width=0.7849999999999999mm,-,/pgfplots/color of colormap=(216)] (layer3 forklift_concept4.east) -- (layer4 forklift_concept5.west);
% % % \draw[line width=0.75mm,-,/pgfplots/color of colormap=(250)] (layer3 forklift_concept4.east) -- (layer4 forklift_concept2.west);
% % \draw[line width=0.9600000000000002mm,-,/pgfplots/color of colormap=(40)] (layer3 forklift_concept3.east) -- (layer4 forklift_concept7.west);
% % \draw[line width=0.8000000000000002mm,-,/pgfplots/color of colormap=(200)] (layer3 forklift_concept3.east) -- (layer4 forklift_concept6.west);
% % \draw[line width=0.9800000000000001mm,-,/pgfplots/color of colormap=(20)] (layer3 forklift_concept3.east) -- (layer4 forklift_concept5.west);
% % \draw[line width=0.9357142857142857mm,-,/pgfplots/color of colormap=(65)] (layer3 forklift_concept3.east) -- (layer4 forklift_concept4.west);
% % \draw[line width=0.8944444444444445mm,-,/pgfplots/color of colormap=(106)] (layer3 forklift_concept3.east) -- (layer4 forklift_concept3.west);
% % % \draw[line width=0.9642857142857144mm,-,/pgfplots/color of colormap=(36)] (layer3 forklift_concept3.east) -- (layer4 forklift_concept2.west);
% % % \draw[line width=0.7357142857142855mm,-,/pgfplots/color of colormap=(265)] (layer3 forklift_concept3.east) -- (layer4 forklift_concept1.west);
% % \draw[line width=0.33461538461538465mm,-,/pgfplots/color of colormap=(666)] (layer2 forklift_concept1.east) -- (layer3 forklift_concept5.west);
% % \draw[line width=0.3386363636363637mm,-,/pgfplots/color of colormap=(662)] (layer2 forklift_concept1.east) -- (layer3 forklift_concept2.west);
% % \draw[line width=0.29999999999999993mm,-,/pgfplots/color of colormap=(701)] (layer2 forklift_concept1.east) -- (layer3 forklift_concept3.west);
% % \draw[line width=0.8550000000000001mm,-,/pgfplots/color of colormap=(145)] (layer3 forklift_concept1.east) -- (layer4 forklift_concept7.west);
% % \draw[line width=0.8333333333333336mm,-,/pgfplots/color of colormap=(167)] (layer3 forklift_concept1.east) -- (layer4 forklift_concept6.west);
% % \draw[line width=0.9400000000000002mm,-,/pgfplots/color of colormap=(60)] (layer3 forklift_concept1.east) -- (layer4 forklift_concept5.west);
% % \draw[line width=0.9214285714285715mm,-,/pgfplots/color of colormap=(79)] (layer3 forklift_concept1.east) -- (layer4 forklift_concept4.west);
% % \draw[line width=0.9055555555555557mm,-,/pgfplots/color of colormap=(95)] (layer3 forklift_concept1.east) -- (layer4 forklift_concept3.west);
% % % \draw[line width=0.9428571428571427mm,-,/pgfplots/color of colormap=(58)] (layer3 forklift_concept1.east) -- (layer4 forklift_concept2.west);
% % \draw[line width=1.0mm,-,/pgfplots/color of colormap=(0)] (layer4 forklift_concept7.east) -- (class forklift.west);
% % \draw[line width=1.0mm,-,/pgfplots/color of colormap=(0)] (layer4 forklift_concept6.east) -- (class forklift.west);
% % \draw[line width=1.0mm,-,/pgfplots/color of colormap=(0)] (layer4 forklift_concept5.east) -- (class forklift.west);
% % \draw[line width=1.0mm,-,/pgfplots/color of colormap=(0)] (layer4 forklift_concept4.east) -- (class forklift.west);
% % \draw[line width=1.0mm,-,/pgfplots/color of colormap=(0)] (layer4 forklift_concept3.east) -- (class forklift.west);
% % % \draw[line width=1.0mm,-,/pgfplots/color of colormap=(0)] (layer4 forklift_concept2.east) -- (class forklift.west);
% % % \draw[line width=0.95mm,-,/pgfplots/color of colormap=(50)] (layer4 forklift_concept1.east) -- (class forklift.west);


% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(636)] ($ (layer1 forklift_concept1.east) - (0.15,0) $ ) -- ( $ (layer2 forklift_concept3.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(489)] ($ (layer1 forklift_concept1.east) - (0.15,0) $ ) -- ( $ (layer2 forklift_concept2.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(635)] ($ (layer2 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept5.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(614)] ($ (layer2 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept2.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(485)] ($ (layer2 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept4.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(727)] ($ (layer2 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept3.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(600)] ($ (layer2 forklift_concept2.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept5.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(604)] ($ (layer2 forklift_concept2.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept1.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(698)] ($ (layer2 forklift_concept2.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept2.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(689)] ($ (layer2 forklift_concept2.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept3.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(603)] ($ (layer1 forklift_concept2.east) - (0.15,0) $ ) -- ( $ (layer2 forklift_concept3.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(452)] ($ (layer1 forklift_concept2.east) - (0.15,0) $ ) -- ( $ (layer2 forklift_concept2.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(90)] ($ (layer3 forklift_concept5.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept7.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(284)] ($ (layer3 forklift_concept5.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept6.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(135)] ($ (layer3 forklift_concept5.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept5.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(215)] ($ (layer3 forklift_concept5.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept4.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(189)] ($ (layer3 forklift_concept5.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept3.west) + (0.15,0) $ );
% % \draw[line width=0.85mm,-,/pgfplots/color of colormap=(150)] (layer3 forklift_concept5.east) -- (layer4 forklift_concept2.west);
% % \draw[line width=0.7499999999999998mm,-,/pgfplots/color of colormap=(251)] (layer3 forklift_concept5.east) -- (layer4 forklift_concept1.west);
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(250)] ($ (layer3 forklift_concept2.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept7.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(367)] ($ (layer3 forklift_concept2.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept6.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(236)] ($ (layer3 forklift_concept2.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept5.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(150)] ($ (layer3 forklift_concept2.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept3.west) + (0.15,0) $ );
% % \draw[line width=0.8142857142857143mm,-,/pgfplots/color of colormap=(186)] (layer3 forklift_concept2.east) -- (layer4 forklift_concept2.west);
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(210)] ($ (layer3 forklift_concept4.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept7.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(216)] ($ (layer3 forklift_concept4.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept5.west) + (0.15,0) $ );
% % \draw[line width=0.75mm,-,/pgfplots/color of colormap=(250)] (layer3 forklift_concept4.east) -- (layer4 forklift_concept2.west);
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(40)] ($ (layer3 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept7.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(200)] ($ (layer3 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept6.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(20)] ($ (layer3 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept5.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(65)] ($ (layer3 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept4.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(106)] ($ (layer3 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept3.west) + (0.15,0) $ );
% % \draw[line width=0.9642857142857144mm,-,/pgfplots/color of colormap=(36)] (layer3 forklift_concept3.east) -- (layer4 forklift_concept2.west);
% % \draw[line width=0.7357142857142855mm,-,/pgfplots/color of colormap=(265)] (layer3 forklift_concept3.east) -- (layer4 forklift_concept1.west);
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(666)] ($ (layer2 forklift_concept1.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept5.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(662)] ($ (layer2 forklift_concept1.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept2.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(701)] ($ (layer2 forklift_concept1.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept3.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(145)] ($ (layer3 forklift_concept1.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept7.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(167)] ($ (layer3 forklift_concept1.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept6.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(60)] ($ (layer3 forklift_concept1.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept5.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(79)] ($ (layer3 forklift_concept1.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept4.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(95)] ($ (layer3 forklift_concept1.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept3.west) + (0.15,0) $ );
% % \draw[line width=0.9428571428571427mm,-,/pgfplots/color of colormap=(58)] (layer3 forklift_concept1.east) -- (layer4 forklift_concept2.west);
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(0)] ($ (layer4 forklift_concept7.east) - (0.15,0) $ ) -- ( $ (class forklift.west) + (0, 0.25) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(0)] ($ (layer4 forklift_concept6.east) - (0.15,0) $ ) -- ( $ (class forklift.west) + (0, 0.25) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(0)] ($ (layer4 forklift_concept5.east) - (0.15,0) $ ) -- ( $ (class forklift.west) + (0, 0.25) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(0)] ($ (layer4 forklift_concept4.east) - (0.15,0) $ ) -- ( $ (class forklift.west) + (0, 0.25) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(0)] ($ (layer4 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (class forklift.west) + (0, 0.25) $ );
% % \draw[line width=1.0mm,-,/pgfplots/color of colormap=(0)] (layer4 forklift_concept2.east) -- (class forklift.west);
% % \draw[line width=0.95mm,-,/pgfplots/color of colormap=(50)] (layer4 forklift_concept1.east) -- (class forklift.west);
% \end{scope}
%     \end{tikzpicture}}
%     \vspace{-0.37cm}
%     % \vfill
%     \hrule
%     % \vfill
%     \vspace{0.04cm}
%     % \vspace{0.02cm}
% % \vspace{0.05cm}
% % \vfill 
%     % \vfill 
%     % \vfill 
%     % \vspace{0.15cm}
% \resizebox{0.48\textwidth}{!}{    
% \begin{tikzpicture}[grow=left,
%         every node/.style = {inner sep=0pt},
% every label/.append style = {label distance=0.5pt, align = center},
%          sibling distance = 5.0em,
%            level 1/.style = {level distance=5em,anchor=east},
%            level 2/.style = {level distance=5em,anchor=east},
%            level 3/.style = {level distance=5em,anchor=east},
%            level 4/.style = {level distance=5em,anchor=east},
%            level 5/.style = {level distance=5em,anchor=east},
%            ]  
% \node[anchor=south,label=Forklift](class forklift)
% {\includegraphics[width=25mm]{images/connectomes/clip_r50_forklift/class forklift.png}}
%     child {node[](layer4 forklift_concept3){\includegraphics[width=17mm]{images/connectomes/clip_r50_forklift/layer4 forklift_concept3.png}} 
%         edge from parent[draw=none]} 
%     child {node[](layer4 forklift_concept1){\includegraphics[width=17mm]{images/connectomes/clip_r50_forklift/layer4 forklift_concept1.png}} 
%         edge from parent[draw=none]} 
%     child {node[](layer4 forklift_concept4){\includegraphics[width=17mm]{images/connectomes/clip_r50_forklift/layer4 forklift_concept4.png}} 
%         edge from parent[draw=none]
%         child {node[](layer3 forklift_concept4){\includegraphics[width=17mm]{images/connectomes/clip_r50_forklift/layer3 forklift_concept4.png}} 
%             edge from parent[draw=none]}
%         child {node[](layer3 forklift_concept3){\includegraphics[width=17mm]{images/connectomes/clip_r50_forklift/layer3 forklift_concept3.png}} 
%             edge from parent[draw=none]} 
%         child {node[](layer3 forklift_concept1) {\includegraphics[width=17mm]{images/connectomes/clip_r50_forklift/layer3 forklift_concept1.png}} 
%             edge from parent[draw=none]
%             child {node[](layer2 forklift_concept4){\includegraphics[width=17mm]{images/connectomes/clip_r50_forklift/layer2 forklift_concept4.png}} 
%             edge from parent[draw=none]}
%             child {node[](layer2 forklift_concept3){\includegraphics[width=17mm]{images/connectomes/clip_r50_forklift/layer2 forklift_concept3.png}} 
%             edge from parent[draw=none]
%                 child {node[](layer1 forklift_concept2){\includegraphics[width=17mm]{images/connectomes/clip_r50_forklift/layer1 forklift_concept2.png}} 
%                 edge from parent[draw=none]}
%                 child {node[](layer1 forklift_concept3){\includegraphics[width=17mm]{images/connectomes/clip_r50_forklift/layer1 forklift_concept3.png}} 
%                 edge from parent[draw=none]}
%                 child {node[](layer1 forklift_concept4){\includegraphics[width=17mm]{images/connectomes/clip_r50_forklift/layer1 forklift_concept4.png}} 
%                 edge from parent[draw=none]}
%                 child {node[](layer1 forklift_concept1){\includegraphics[width=17mm]{images/connectomes/clip_r50_forklift/layer1 forklift_concept1.png}} 
%                 edge from parent[draw=none]}
%             }
%             child {node[](layer2 forklift_concept1){\includegraphics[width=17mm]{images/connectomes/clip_r50_forklift/layer2 forklift_concept1.png}} 
%             edge from parent[draw=none]}
%             }
%         child {node[](layer3 forklift_concept6){\includegraphics[width=17mm]{images/connectomes/clip_r50_forklift/layer3 forklift_concept6.png}} 
%             edge from parent[draw=none]} 
%         child {node[](layer3 forklift_concept5){\includegraphics[width=17mm]{images/connectomes/clip_r50_forklift/layer3 forklift_concept5.png}} 
%             edge from parent[draw=none]}
%             } 
%     child {node[](layer4 forklift_concept5){\includegraphics[width=17mm]{images/connectomes/clip_r50_forklift/layer4 forklift_concept5.png}} edge from parent[draw=none]
%             }
%     child {node[](layer4 forklift_concept2){\includegraphics[width=17mm]{images/connectomes/clip_r50_forklift/layer4 forklift_concept2.png}} edge from parent[draw=none]
%             };
% % ARROWS
% \begin{scope}[on background layer]
% % \draw[line width=0.5296875mm,-,/pgfplots/color of colormap=(471)] (layer1 forklift_concept2.east) -- (layer2 forklift_concept4.west);
% % % \draw[line width=0.36571428571428577mm,-,/pgfplots/color of colormap=(635)] (layer1 forklift_concept2.east) -- (layer2 forklift_concept6.west);
% % \draw[line width=0.46153846153846156mm,-,/pgfplots/color of colormap=(539)] (layer1 forklift_concept2.east) -- (layer2 forklift_concept3.west);
% % \draw[line width=0.36800000000000016mm,-,/pgfplots/color of colormap=(632)] (layer1 forklift_concept2.east) -- (layer2 forklift_concept1.west);
% % % \draw[line width=0.3999999999999998mm,-,/pgfplots/color of colormap=(601)] (layer1 forklift_concept2.east) -- (layer2 forklift_concept5.west);
% % \draw[line width=0.6423076923076921mm,-,/pgfplots/color of colormap=(358)] (layer2 forklift_concept4.east) -- (layer3 forklift_concept4.west);
% % \draw[line width=0.6230769230769229mm,-,/pgfplots/color of colormap=(377)] (layer2 forklift_concept4.east) -- (layer3 forklift_concept3.west);
% % \draw[line width=0.5617647058823528mm,-,/pgfplots/color of colormap=(439)] (layer2 forklift_concept4.east) -- (layer3 forklift_concept1.west);
% % \draw[line width=0.538235294117647mm,-,/pgfplots/color of colormap=(462)] (layer2 forklift_concept4.east) -- (layer3 forklift_concept6.west);
% % % \draw[line width=0.7442307692307691mm,-,/pgfplots/color of colormap=(256)] (layer2 forklift_concept4.east) -- (layer3 forklift_concept2.west);
% % \draw[line width=0.43571428571428583mm,-,/pgfplots/color of colormap=(565)] (layer2 forklift_concept4.east) -- (layer3 forklift_concept5.west);
% % \draw[line width=0.5557692307692307mm,-,/pgfplots/color of colormap=(445)] (layer2 forklift_concept3.east) -- (layer3 forklift_concept4.west);
% % \draw[line width=0.5235294117647059mm,-,/pgfplots/color of colormap=(477)] (layer2 forklift_concept3.east) -- (layer3 forklift_concept1.west);
% % \draw[line width=0.4882352941176471mm,-,/pgfplots/color of colormap=(512)] (layer2 forklift_concept3.east) -- (layer3 forklift_concept6.west);
% % % \draw[line width=0.6057692307692306mm,-,/pgfplots/color of colormap=(395)] (layer2 forklift_concept3.east) -- (layer3 forklift_concept2.west);
% % \draw[line width=0.6076923076923075mm,-,/pgfplots/color of colormap=(393)] (layer2 forklift_concept1.east) -- (layer3 forklift_concept4.west);
% % \draw[line width=0.5205882352941177mm,-,/pgfplots/color of colormap=(480)] (layer2 forklift_concept1.east) -- (layer3 forklift_concept1.west);
% % \draw[line width=0.47352941176470587mm,-,/pgfplots/color of colormap=(527)] (layer2 forklift_concept1.east) -- (layer3 forklift_concept6.west);
% % % \draw[line width=0.6673076923076922mm,-,/pgfplots/color of colormap=(333)] (layer2 forklift_concept1.east) -- (layer3 forklift_concept2.west);
% % % \draw[line width=0.42051282051282063mm,-,/pgfplots/color of colormap=(580)] (layer1 forklift_concept3.east) -- (layer2 forklift_concept2.west);
% % \draw[line width=0.5mm,-,/pgfplots/color of colormap=(500)] (layer1 forklift_concept3.east) -- (layer2 forklift_concept4.west);
% % % \draw[line width=0.3971428571428573mm,-,/pgfplots/color of colormap=(603)] (layer1 forklift_concept3.east) -- (layer2 forklift_concept6.west);
% % \draw[line width=0.4666666666666667mm,-,/pgfplots/color of colormap=(534)] (layer1 forklift_concept3.east) -- (layer2 forklift_concept3.west);
% % \draw[line width=0.3560000000000001mm,-,/pgfplots/color of colormap=(644)] (layer1 forklift_concept3.east) -- (layer2 forklift_concept1.west);
% % % \draw[line width=0.4048387096774192mm,-,/pgfplots/color of colormap=(596)] (layer1 forklift_concept3.east) -- (layer2 forklift_concept5.west);
% % % \draw[line width=0.33571428571428563mm,-,/pgfplots/color of colormap=(665)] (layer1 forklift_concept4.east) -- (layer2 forklift_concept6.west);
% % \draw[line width=0.3880000000000001mm,-,/pgfplots/color of colormap=(612)] (layer1 forklift_concept4.east) -- (layer2 forklift_concept1.west);
% % % \draw[line width=0.40967741935483853mm,-,/pgfplots/color of colormap=(591)] (layer1 forklift_concept4.east) -- (layer2 forklift_concept5.west);
% % % \draw[line width=0.3794871794871795mm,-,/pgfplots/color of colormap=(621)] (layer1 forklift_concept1.east) -- (layer2 forklift_concept2.west);
% % \draw[line width=0.5046875mm,-,/pgfplots/color of colormap=(496)] (layer1 forklift_concept1.east) -- (layer2 forklift_concept4.west);
% % % \draw[line width=0.39857142857142874mm,-,/pgfplots/color of colormap=(602)] (layer1 forklift_concept1.east) -- (layer2 forklift_concept6.west);
% % \draw[line width=0.3720000000000001mm,-,/pgfplots/color of colormap=(628)] (layer1 forklift_concept1.east) -- (layer2 forklift_concept1.west);
% % % \draw[line width=0.4258064516129031mm,-,/pgfplots/color of colormap=(575)] (layer1 forklift_concept1.east) -- (layer2 forklift_concept5.west);
% % \draw[line width=0.60625mm,-,/pgfplots/color of colormap=(394)] (layer3 forklift_concept4.east) -- (layer4 forklift_concept3.west);
% % \draw[line width=0.48571428571428565mm,-,/pgfplots/color of colormap=(515)] (layer3 forklift_concept3.east) -- (layer4 forklift_concept1.west);
% % \draw[line width=0.7mm,-,/pgfplots/color of colormap=(300)] (layer3 forklift_concept3.east) -- (layer4 forklift_concept3.west);
% % \draw[line width=0.5928571428571427mm,-,/pgfplots/color of colormap=(408)] (layer3 forklift_concept1.east) -- (layer4 forklift_concept4.west);
% % \draw[line width=0.68125mm,-,/pgfplots/color of colormap=(319)] (layer3 forklift_concept1.east) -- (layer4 forklift_concept3.west);
% % \draw[line width=0.46428571428571425mm,-,/pgfplots/color of colormap=(536)] (layer3 forklift_concept6.east) -- (layer4 forklift_concept5.west);
% % \draw[line width=0.7375mm,-,/pgfplots/color of colormap=(263)] (layer3 forklift_concept6.east) -- (layer4 forklift_concept3.west);
% % % \draw[line width=0.66875mm,-,/pgfplots/color of colormap=(332)] (layer3 forklift_concept2.east) -- (layer4 forklift_concept3.west);
% % \draw[line width=0.4357142857142858mm,-,/pgfplots/color of colormap=(565)] (layer3 forklift_concept5.east) -- (layer4 forklift_concept5.west);
% % \draw[line width=0.5375mm,-,/pgfplots/color of colormap=(463)] (layer3 forklift_concept5.east) -- (layer4 forklift_concept2.west);
% % \draw[line width=0.607142857142857mm,-,/pgfplots/color of colormap=(393)] (layer3 forklift_concept5.east) -- (layer4 forklift_concept4.west);
% % \draw[line width=0.58125mm,-,/pgfplots/color of colormap=(419)] (layer3 forklift_concept5.east) -- (layer4 forklift_concept3.west);
% % \draw[line width=0.28300000000000003mm,-,/pgfplots/color of colormap=(717)] (layer4 forklift_concept3.east) -- (class forklift.west);
% % \draw[line width=0.28500000000000003mm,-,/pgfplots/color of colormap=(715)] (layer4 forklift_concept4.east) -- (class forklift.west);
% % \draw[line width=0.7500000000000001mm,-,/pgfplots/color of colormap=(250)] (layer4 forklift_concept5.east) -- (class forklift.west);
% % \draw[line width=0.742mm,-,/pgfplots/color of colormap=(258)] (layer4 forklift_concept2.east) -- (class forklift.west);

% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(471)] ( $ (layer1 forklift_concept2.east) - (0.15,0) $ ) -- ( $ (layer2 forklift_concept4.west) + (0.15,0) $ );
% % \draw[line width=0.36571428571428577mm,-,/pgfplots/color of colormap=(635)] (layer1 forklift_concept2.east) -- (layer2 forklift_concept6.west);
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(539)] ( $ (layer1 forklift_concept2.east) - (0.15,0) $ ) -- ( $ (layer2 forklift_concept3.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(632)] ( $ (layer1 forklift_concept2.east) - (0.15,0) $ ) -- ( $ (layer2 forklift_concept1.west) + (0.15,0) $ );
% % \draw[line width=0.3999999999999998mm,-,/pgfplots/color of colormap=(601)] (layer1 forklift_concept2.east) -- (layer2 forklift_concept5.west);
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(358)] ( $ (layer2 forklift_concept4.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept4.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(377)] ( $ (layer2 forklift_concept4.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept3.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(439)] ( $ (layer2 forklift_concept4.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept1.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(462)] ( $ (layer2 forklift_concept4.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept6.west) + (0.15,0) $ );
% % \draw[line width=0.7442307692307691mm,-,/pgfplots/color of colormap=(256)] (layer2 forklift_concept4.east) -- (layer3 forklift_concept2.west);
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(565)] ( $ (layer2 forklift_concept4.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept5.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(445)] ( $ (layer2 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept4.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(477)] ( $ (layer2 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept1.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(512)] ( $ (layer2 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept6.west) + (0.15,0) $ );
% % \draw[line width=0.6057692307692306mm,-,/pgfplots/color of colormap=(395)] (layer2 forklift_concept3.east) -- (layer3 forklift_concept2.west);
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(393)] ( $ (layer2 forklift_concept1.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept4.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(480)] ( $ (layer2 forklift_concept1.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept1.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(527)] ( $ (layer2 forklift_concept1.east) - (0.15,0) $ ) -- ( $ (layer3 forklift_concept6.west) + (0.15,0) $ );
% % \draw[line width=0.6673076923076922mm,-,/pgfplots/color of colormap=(333)] (layer2 forklift_concept1.east) -- (layer3 forklift_concept2.west);
% % \draw[line width=0.42051282051282063mm,-,/pgfplots/color of colormap=(580)] (layer1 forklift_concept3.east) -- (layer2 forklift_concept2.west);
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(500)] ( $ (layer1 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (layer2 forklift_concept4.west) + (0.15,0) $);
% % \draw[line width=0.3971428571428573mm,-,/pgfplots/color of colormap=(603)] (layer1 forklift_concept3.east) -- (layer2 forklift_concept6.west);
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(534)] ( $ (layer1 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (layer2 forklift_concept3.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(644)] ( $ (layer1 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (layer2 forklift_concept1.west) + (0.15,0) $ );
% % \draw[line width=0.4048387096774192mm,-,/pgfplots/color of colormap=(596)] (layer1 forklift_concept3.east) -- (layer2 forklift_concept5.west);
% % \draw[line width=0.33571428571428563mm,-,/pgfplots/color of colormap=(665)] (layer1 forklift_concept4.east) -- (layer2 forklift_concept6.west);
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(612)] ( $ (layer1 forklift_concept4.east) - (0.15,0) $ ) -- ( $ (layer2 forklift_concept1.west) + (0.15,0) $ );
% % \draw[line width=0.40967741935483853mm,-,/pgfplots/color of colormap=(591)] (layer1 forklift_concept4.east) -- (layer2 forklift_concept5.west);
% % \draw[line width=0.3794871794871795mm,-,/pgfplots/color of colormap=(621)] (layer1 forklift_concept1.east) -- (layer2 forklift_concept2.west);
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(496)] ( $ (layer1 forklift_concept1.east) - (0.15,0) $ ) -- ( $ (layer2 forklift_concept4.west) + (0.15,0) $ );
% % \draw[line width=0.39857142857142874mm,-,/pgfplots/color of colormap=(602)] (layer1 forklift_concept1.east) -- (layer2 forklift_concept6.west);
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(628)] ( $ (layer1 forklift_concept1.east) - (0.15,0) $ ) -- ( $ (layer2 forklift_concept1.west) + (0.15,0) $ );
% % \draw[line width=0.4258064516129031mm,-,/pgfplots/color of colormap=(575)] (layer1 forklift_concept1.east) -- (layer2 forklift_concept5.west);
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(394)] ( $ (layer3 forklift_concept4.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept3.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(515)] ( $ (layer3 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept1.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(300)] ( $ (layer3 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept3.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(408)] ( $ (layer3 forklift_concept1.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept4.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(319)] ( $ (layer3 forklift_concept1.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept3.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(536)] ( $ (layer3 forklift_concept6.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept5.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(263)] ( $ (layer3 forklift_concept6.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept3.west) + (0.15,0) $ );
% % \draw[line width=0.66875mm,-,/pgfplots/color of colormap=(332)] (layer3 forklift_concept2.east) -- (layer4 forklift_concept3.west);
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(565)] ( $ (layer3 forklift_concept5.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept5.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(463)] ( $ (layer3 forklift_concept5.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept2.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(393)] ( $ (layer3 forklift_concept5.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept4.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(419)] ( $ (layer3 forklift_concept5.east) - (0.15,0) $ ) -- ( $ (layer4 forklift_concept3.west) + (0.15,0) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(717)] ( $ (layer4 forklift_concept3.east) - (0.15,0) $ ) -- ( $ (class forklift.west) + (0, 0.25) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(715)] ( $ (layer4 forklift_concept4.east) - (0.15,0) $ ) -- ( $ (class forklift.west) + (0, 0.25) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(250)] ( $ (layer4 forklift_concept5.east) - (0.15,0) $ ) -- ( $ (class forklift.west) + (0, 0.25) $ );
% \draw[line width=0.6mm,-,/pgfplots/color of colormap=(258)] ( $ (layer4 forklift_concept2.east) - (0.15,0) $ ) -- ( $ (class forklift.west) + (0, 0.25) $ );
% \end{scope}
%     \end{tikzpicture}
% } \vspace{-0.75cm}
% \caption{\textcolor{red}{A comparison of ResNet50 VCCs   
% %(top) ResNet50~\cite{he2016deep} 
% trained with (top) ImageNet~\cite{deng2009imagenet} and (bottom) contrastive image-language pretraining~\cite{radford2021learning} (CLIP). Each VCC shows the same four layers consisting of ResNet residual blocks.} %in ResNet architectures.
% % \textcolor{red}{Need better separation between top and bottom.}
% }
% \label{fig:clip_r50_vcc_compare} \vspace{-14pt}
% \end{figure}


% \input{sec/4_experiments_AllLayer}

